Bound Analysis of Imperative Programs with the Size-change Abstraction (extended version)

The size-change abstraction (SCA) is an important program abstraction for termination analysis, which has been successfully implemented in many tools for functional and logic programs. In this paper, we demonstrate that SCA is also a highly effective abstract domain for the bound analysis of imperative programs. We have implemented a bound analysis tool based on SCA for imperative programs. We abstract programs in a pathwise and context dependent manner, which enables our tool to analyze real-world programs effectively. Our work shows that SCA captures many of the essential ideas of previous termination and bound analysis and goes beyond in a conceptually simpler framework.

==> include/abstraction.tex <==
\svnid{$Id$}

\vspace{-1.3cm}

\section{Computing Transition Systems}
\label{sec:abstraction}

\vspace{-0.2cm}

%By following these approaches we assume that programs always have a special \emph{start} and \emph{end location}, which we denote by $\locstart$ and $\locend$, and that $\locstart$ has no incoming edges and $\locend$ has no outgoing edges.
%Our goal is to transform every program into an SCS that overapproximates the transition relation between $\locstart$ and $\locend$.

%\begin{definition}
%  Let $G = (V,E)$ be a directed graph.
%  A strongly connected component \emph{SCC} $S \subseteq V$ is a set of vertices such that for every pair of vertices $s_1,s_2 \in S$ there is a path from $s_1$ to $s_2$ and there is no such path from $s_1$ to $s_2$ that uses a vertex not in $S$.
%  A \emph{loop header} of an SCC $S$ is a vertex $s \in S$ such that there is a vertex $v \in V \setminus S$ with $(v,s) \in E$.
%  A loop header $s \in S$ is \emph{unique}, if it holds that $v_1,v_2 \in V \setminus S$ and $(v_1,s), (v_2,s) \in E$ imply $v_1 = v_2$.
%  A backedge is an edge $(v,s)$ such that $s$ is an entrance point of an SCC.
%\end{definition}
%Note that according to our definition all SCCs are maximal.
%
%\begin{definition}[Reducibility]
%  A directed graph is \emph{reducible}, if
%  \begin{itemize}
%  \item it does not have an SCC, or
%  \item every SCC has a unique entrance point, and after deleting all backedges we get a reducible graph.
%  \end{itemize}
%\end{definition}

In this section we describe our algorithm for computing transition systems.
We first present the actual algorithm, and then discuss specific characteristics.
%
The function $\TransSys$ in Algorithm~\ref{alg:transitionSystem}
takes as input a program  $\prog = (\locs,\edges)$ and a location $\loc \in \locs$ and computes a transition system for $\prog|_\loc$, cf.~Theorem~\ref{thm:TransSys-Correctness} below.
The key ideas of Algorithm~\ref{alg:transitionSystem} are
(1) to summarize inner loops disjunctively by transition invariants computed with SCA, and
(2) to enumerate all cycle-free paths for pathwise analysis.
% and use these paths and the summaries of the inner loops for pathwise analysis (discussed in Subsection~\ref{subsec:pathwise-analysis}.).%, which are implemented in the two $\mathtt{foreach}$-loops.
%Next we describe Algorithm~\ref{alg:transitionSystem} in detail.
Note that for loop summarization the algorithm is recursively invoked.
\final{We give an example for the application of Algorithm~\ref{alg:transitionSystem} to Example~\ref{ex:abstraction} in the extended version.}
\full{We give an example for the application of Algorithm~\ref{alg:transitionSystem} to Example~\ref{ex:abstraction} in Section~\ref{app:alg1example} of the appendix.}


\vspace{-0.2cm}
\paragraph{\bfseries Loop Summarization.}
In the first $\mathtt{foreach}$-loop, Algorithm~\ref{alg:transitionSystem} iterates over all nested loops of $\prog$ w.r.t. $\loc$.
A loop $\looop$ of $\prog$ is a nested loop w.r.t. $\loc$, if it is strongly connected to $\loc$ but does not contain $\loc$, and if there is no loop with the same properties that strictly contains $\looop$.
% can be reached from $\loc$ and from which $\loc$ is reachable.
Let $\looop$ be a nested loop of $\prog$ w.r.t. $\loc$ and let $\header$ be its header.
(We assume that the program is reducible, see discussion below.)
$\TransSys$ calls itself recursively to compute a transition system $\transinv$ for $\looop|_\header$.
%Next, procedure $\mathtt{unroll}$, which we present in Subsection~\ref{subsec:unrolling}, returns an unrolling $(\mathit{next},\mathit{exit})$ of $\transinv$, where the transition sets $\mathit{next}$ and $\mathit{exit}$ satisfy the equation $\mathit{next}^* \circ \mathit{exit} = \transinv^*$.
%\hv{Role and definition of unrolling unclear here.}
%\textbf{TODO:} Be careful with sets and sets of sets.

In statement $\closure := \gamma(\alpha(\transinv)^*)$,
$\alpha(\transinv)$ size-change abstracts $\transinv$ to an SCR set, $\alpha(\transinv)^*$ computes the transitive hull of this SCR set, and $\gamma(\alpha(\transinv)^*)$ concretizes the abstract transitive hull to a transition set, which is then assigned to $\closure$.
%Because of Theorem~\ref{thm:soundness}, $\closure \circ exit$ is a transition invariant for $\looop|_\header$.
Algorithm~\ref{alg:transitionSystem} stores $\closure$ in the array $\Summary$, which is a transition invariant for $\looop|_\header$ by the soundness of SCA as stated in Theorem~\ref{thm:soundness}.

After the first $\mathtt{foreach}$-loop, Algorithm~\ref{alg:transitionSystem} has summarized all inner loops, not only the nested loops, because the recursive calls reaches all nesting levels.
For each inner loop $\looop$ with header $\header$ a transition invariant for $\looop|_\header$ has been stored at $\Summary[\header]$.
Summaries of inner loops are visible to all outer loops, because the array $\Summary$ is a global variable.
\vspace{-0.2cm}
\paragraph{\bfseries Pathwise Analysis.}
In the second $\mathtt{foreach}$-loop, Algorithm~\ref{alg:transitionSystem} iterates over all cycle-free paths of $\prog$ with start and end location $\loc$.
Let $\paath = \loc \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \cdots \loc_k \xrightarrow{\trn_k} \loc$ be such a cycle-free path.
The expression $\ITE(\IsHeader(\loc_i),\Summary[\loc_i], \{Id\})$ evaluates to $\Summary[\loc_i]$ for each location $\loc_i$, if $\loc_i$ is the header of an inner loop $\looop_i$, and evaluates to the transition set $\{Id\}$, which contains only the identity relation over the program states, else.
Algorithm~\ref{alg:transitionSystem} computes the set $\transinv_\paath = \{\trn_0\} \circ$\\ $\ITE(\IsHeader(\loc_1),\Summary[\loc_1], \{Id\}) \circ \{\trn_1\} \circ \ITE(\IsHeader(\loc_2),\Summary[\loc_2], \{Id\})$ \\
$ \circ \{\trn_2\} \circ \cdots \circ \ITE(\IsHeader(\loc_k),\Summary[\loc_k], \{Id\}) \circ \{\trn_k\}$, which is an overapproximation of the contraction of $\paath$, where the summaries of the inner loops $\looop_i$ are inserted at their headers $\loc_i$.
The transition set $\transinv_\paath$ overapproximates all paths starting and ending in $\loc$ that iterate arbitrarily often through inner loops along $\paath$, because for every loop $\looop_i$ the transition set $\Summary[\loc_i]$ overapproximates all paths starting and ending in $\loc_i$ that iterate arbitrarily often through $\looop_i$ (as $\Summary[\loc_i]$ is a transition invariant for $\looop_i|_{\loc_i}$).
%Overapproximates means here: is a transition system for the union of the transition relations of all paths that...
%is a transition system for the union of the transition relations $\rel(\paath)$ of all paths $\paath$ that...
Algorithm~\ref{alg:transitionSystem} returns the union $\bigcup_{\text{cycle-free path } \paath \in \mathtt{paths}(\prog,\loc)} \transinv_\paath$ of all those transition sets $\transinv_\paath$.
%of all cycle-free path $\paath \in \mathtt{paths}(\prog,\loc)$.
%$ = \TransSys(\prog,\loc)$ as transition system for $\prog|_\loc$.

\begin{theorem}
\label{thm:TransSys-Correctness}
  Algorithm~\ref{alg:transitionSystem} computes a transition system $\TransSys(\prog,\loc)$ for $\prog|_\loc$.
\end{theorem}
\begin{proof}[Sketch]
%We show that for every simple path $\paath \in \mathtt{paths}(\prog,\loc)}$ there is a cycle-free path $\paath \in \mathtt{paths}(\prog,\loc)$ such that $\transinv_\paath$ is a transition system for $\rel(\paath^\prime)$.
%This is sufficient because of $\prog|_\loc = \bigcup_{\text{simple } \paath \in \mathtt{paths}(\prog,\loc)} \rel(\paath)$ and $\TransSys(\prog,\loc) = \bigcup_{\text{cycle-free path } \paath \in \mathtt{paths}(\prog,\loc)} \transinv_\paath$.
Let $\paath^\prime \in \mathtt{paths}(\prog,\loc)$ be a simple path.
We obtain a cycle-free path $\paath \in \mathtt{paths}(\prog,\loc)$ from $\paath^\prime$ by deleting all iterations through inner loops of $(\prog,\loc)$ from $\paath^\prime$.
The transition set $\transinv_\paath$ overapproximates all paths starting and ending in $\loc$ that iterate arbitrarily often through inner loops of $(\prog,\loc)$ along $\paath$.
As $\paath^\prime$ iterates through inner loops of $(\prog,\loc)$ along $\paath$ we have $\rel(\paath) \subseteq \bigcup \transinv_\paath$.
%Thus $\transinv_\paath$ is a transition system for $\rel(\paath^\prime)$.
\end{proof}

\paragraph{Implementation.}
We use conjunctions of formulae to represent individual transitions.
This allows us to implement the concatenation of transition relations by conjoining their formulae and introducing existential quantifiers for the intermediate variables.
We detect empty transition relations by asking an SMT solver whether their corresponding formulae are satisfiable.
We use these emptiness checks at several points during the analysis to reduce the number of transition relations.

\noindent Algorithm~\ref{alg:transitionSystem} may exponentially blow up in size because of the enumeration of all cycle-free paths and the computation of transitive hulls of inner loops.
We observed in our experiments that by first extracting norms from the program under scrutiny and then slicing the program w.r.t. these norms before continuing with the analysis normally results into programs small enough for making our analysis feasible.
\vspace{-0.2cm}
\paragraph{Irreducible programs.}
Algorithm~\ref{alg:transitionSystem} refers to loop headers,
and thus implicitly assumes that loops are reducible.
(Recall that in a reducible program each SCC has a unique entry point called the header.)
We have formulated Algorithm~\ref{alg:transitionSystem} in this way to make clear how it exploits the looping structure of imperative programs.
However, Algorithm~\ref{alg:transitionSystem} can be easily extended to irreducible loops by a case distinction on the (potentially multiple) entry points of SCCs.
%In practice imperative programs are reducible or have SCCs with only a few entry points.
%Therefore Algorithm~\ref{alg:transitionSystem} exploits the looping structure of imperative programs.



%\input{include/transformation}
\vspace{-0.3cm}
\subsection{Disjunctiveness in Algorithm 1}
\vspace{-0.1cm}

Disjunctiveness is crucial for bound analysis.
We have given two examples for this fact in Section~\ref{section:example} and refer the reader for further examples to~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07,conf/lics/PodelskiR04}.
\final{We emphasize that our analysis can handle {\em all examples} of these publications.}
\full{We emphasize that our analysis can handle {\em all examples} of these publications, and give a detailed comparison with them in Section~\ref{sec:comparison}}.
Our analysis is disjunctive in two ways:

% We approximate the disjunction introduced by looping.
(1) \emph{We summarize inner loops disjunctively.}
Given a transition system $\transinv$ for some inner loop $\looop$, we want to summarize $\looop$ by a transition invariant.
The most precise transition invariant $\transinv^* = \{Id\} \cup \transinv \cup \transinv^2 \cup \transinv^3 \cup \cdots$ introduces infinitely many disjunctions and is not computable in general.
In contrast to this the abstract transitive hull $\alpha(\transinv)^* = \alpha(\{Id\}) \cup \alpha(\transinv) \cup \alpha(\transinv)^2 \cup \alpha(\transinv)^3 \cup \cdots$ has only finitely many disjunctions and is effectively computable.
This allows us to overapproximate the infinite disjunction $\transinv^*$ by the finite disjunction $\gamma(\alpha(\transinv)^*)$.

We underline that the need for disjunctive summaries of inner loops in the bound analysis is a major motivation for SCA, as it allows us to compute disjunctive transitive hulls naturally, cf.~definition and discussion in Section~\ref{subsec:scs}.

% We approximate the disjunction introduced by branching.
(2) \emph{We summarize local transition relations disjunctively.}
Given a program $\prog = (\locs,\edges)$ and location $\loc \in \locs$, we want to compute a transition system for $\prog|_\loc$.
For a cycle-free path $\paath \in \mathtt{paths}(\prog,\loc)$ the transition set $\transinv_\paath$ computed in Algorithm~\ref{alg:transitionSystem} overapproximates all simple paths in $\mathtt{paths}(\prog,\loc)$ that iterate through inner loops along $\paath$.
As all $\transinv_\paath$ are sets, the set union $\bigcup_{\text{cycle-free path } \paath \in \mathtt{paths}(\prog,\loc)} \transinv_\paath$ is a disjunctive summarization of all $\transinv_\paath$ that keeps the information from different paths separated.
%
This is important for our analysis which relies on the observation that monotonic changes of norms can be observed along single paths from loop header back to the header.

\vspace{-0.3cm}
\subsection{Pathwise Analysis in Algorithm 1}
\label{subsec:pathwise-analysis}
\vspace{-0.1cm}
%In this section, we discuss a specific aspect of Algorithm~\ref{alg:transitionSystem}, namely its pathwise analysis.

It is well-known that analyzing large program parts jointly improves the precision of static analyses, e.g.~\cite{conf/popl/ColbyL96}.
Owing to the progress in SMT solvers this idea has recently seen renewed interested by static analyses such as abstract interpretation~\cite{conf/popl/Monniaux09} and software model checking~\cite{conf/fmcad/BeyerCGKS09}, which use SMT solvers for abstracting large blocks of straight-line code jointly to increase the precision of the analysis.
%A static analysis is more precise by abstracting large pieces of code, e.g., blocks rather than single statements.
%With Algorithm~\ref{alg:transitionSystem} we present a new method for %abstracting large program parts jointly with the help of SMT solvers, which we %call \emph{pathwise-analysis}.

We call the analyses of~\cite{conf/popl/Monniaux09,conf/fmcad/BeyerCGKS09} and classical SCA~\cite{conf/popl/LeeJB01,mcs-integers} \emph{blockwise}, because they do joint abstraction only for loop-free program parts.
In contrast, our \emph{pathwise analysis} abstracts complete paths at once:
Algorithm~\ref{alg:transitionSystem} enumerates all cycle-free paths from loop header to loop header and inserts summaries for inner loops on these paths.
These paths are then abstracted jointly in a subsequent loop summarization or bound computation.
In this way our pathwise analysis is strictly more precise than blockwise analysis.
\final{We illustrate this issue on Example~\ref{ex:abstraction} for SCA the extended version of this paper.}
\full{We illustrate this difference in precision on Example~\ref{ex:abstraction} in Section~\ref{sec:blockpath} of the appendix.}

%We compare the pathwise and blockwise use of SCA in the following.


%We illustrate the difference between block- and pathwise SCA on the program $\prog = (\{\loc,\loc^\prime\}, \{\loc \xrightarrow{\trn_1} \loc^\prime, \loc^\prime \xrightarrow{\trn_2} \loc^\prime, \loc^\prime \xrightarrow{\trn_3} \loc\})$, where $\trn_1 \equiv i^\prime = i + 1, \trn_2 \equiv i^\prime = i + 1, \trn_3 \equiv i^\prime = i - 1$.
%Note that $\prog$ has an inner loop $\looop = (\{\loc^\prime\}, \{\loc^\prime \xrightarrow{\trn_2} \loc^\prime\})$.
%Assume we want to compute a transition invariant for $\prog|_\loc$.
%Choosing $\norms = \{i\}$, we have $\alpha(\trn_1) = i < i^\prime$, $\alpha(\trn_2) = i < i^\prime$, $\alpha(\trn_3) = i > i^\prime$, and $\{i < i^\prime\}^* = \{i \le i^\prime\}$.
%
%Because of the inner loop $\looop$, $\prog$ has exactly three blocks, which coincide with the edges of $\prog$.
%Classical SCA first abstracts these three blocks to SCRs, and then enumerates
%all paths from $\loc$ to $\loc$ in the abstract by one transitive hull computation $(\{\alpha(\trn_1)\} \circ \{\alpha(\trn_2)\}^* \circ \{\alpha(\trn_3)\})^* = \{ i < i^\prime \circ i < i^\prime \circ i > i^\prime, i < i^\prime \circ i = i^\prime \circ i > i^\prime\}^* = \{true\}^* = \{true\}$. (Note there is a nested transitive hull expression for the inner loop.)
%Note that blockwise SCA cannot prove that $i$ never decreases.
%
%In pathwise SCA we first compute the transition system $\transinv_{\loc^\prime} = \{i^\prime = i + 1\}$ for $\looop|_{\loc^\prime}$.
%Then we compute $\alpha(\transinv_{\loc^\prime})^* = \{i < i^\prime\}^* = \{i \le i^\prime\}$.
%We get the transition invariant $\Summary[\loc^\prime] = \{i \le i^\prime i^\prime\}$ for $\looop|_{\loc^\prime}$.
%Then we enumerate all paths of the outer loop using the summary of the inner loop.
%We get the transition system $\transinv_\loc = \{\trn_1\} \circ \Summary[\loc^\prime] \circ \{\trn_3\} = \{ i^\prime = i + 1 \circ i \le i^\prime \circ i^\prime = i - 1\} = \{i^\prime \ge i+1\}$ for $\prog|_\loc$.
%Note that the transitive hull of the size-change abstraction $\alpha(\transinv_\loc)^* = \{i \le i^\prime\}^* = \{i \le i^\prime\}$ of $\transinv_\loc$ can prove that $i$ never decreases.

%Our contribution is to recognize the importance of pathwise SCA for imperative programs.
%We believe that pathwise abstraction can also successfully be used with other static analyses.

Parsers are a natural class of programs which illustrate the need for pathwise analysis.
In our experiments we observed that many parsers increase an index while scanning the input stream and use lookahead to detect which token comes next.
As in Example~\ref{ex:abstraction}, lookaheads may temporarily decrease the index.
Pathwise abstraction is crucial to reason about the program progress with SCA.

%The inner loop uses the same index $i$ to skip over consecutive spaces in the input.
%$i$ is increased by seven before the inner loop and decreased by one afterwards depending on whether the character {\tt chPtr[i]} equals `='.
%\begin{example}
%\label{ex:parse}
%\begin{verbatim}
%void parse (char* chPtr, int length) {
%  int i = 0;
%  while(i < length) {
%    i += 7;
%    while ((i < length) && (chPtr[i] == ' '))
%      i++;
%    if (chPtr[i] != '=')
%      i--;
%}
%\end{verbatim}
%\end{example}
%The number of iterations of the main loop is bounded by $\mathit{length}$ because $i$ is always increased and $i \le \mathit{length}$ is an invariant at the loop header.
%The number of iterations of the inner loop is as well bounded by $\mathit{length}$ because it uses the same counter $i$ as the outer loop and $i \le \mathit{length}$ is an invariant at the loop header.

%Blockwise SCA abstracts the path from the for to the while loop to the SCR $i < i^\prime$, the transitive hull of the while loop to $i \le i^\prime$, and the path from the while loop back to the for loop to $i > i^\prime$.
%
%We consider the cycle-free path
%%$\paath = \loc \xrightarrow{\mathtt{assume}(i < length)} \loc_1 \xrightarrow{i += 7}  \loc_2 \xrightarrow{\mathtt{assume}(\neg(i < length) \wedge (chPtr[i] = \text{' '}))}  \loc_3 \xrightarrow{\mathtt{assume}(chPtr[i] != \text{'='})} \loc_4 \xrightarrow{i--} \loc$
%$\paath = \loc \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \loc_2 \xrightarrow{\trn_2}  \loc_3 \xrightarrow{\trn_3} \loc_4 \xrightarrow{\trn_4} \loc$, where $\trn_0 = \mathtt{assume(i < length)}$, $\trn_1 = \mathtt{i += 7}$, $\trn_2 = \mathtt{assume(chPtr[i] \neq \text{' '}))}$, $\trn_3 = \mathtt{assume(chPtr[i] \neq \text{'='}))}$, $\trn_4 = \mathtt{i--}$, and assume that $\paath$ does not visit further locations.
%
%Algorithm~\ref{alg:transitionSystem} has already computed the summary $\Summary[\loc_2] = \{i \le i^\prime\}$, which is a transition invariant for the nested while loop.
%Algorithm~\ref{alg:transitionSystem} computes the transition set $\transinv_\paath = \{i \}$
%$\paath$ is part of the union $\bigcup_{\text{cycle-free path } \paath \in \mathtt{paths}(\prog,\loc)} \transinv_\paath$.







==> include/algorithm.tex <==
\svnid{$Id$}
\vspace{-0.3cm}
\section{Main Steps of our Analysis}
\label{sec:overview}
\vspace{-0.3cm}
Let $\prog = (\locs,\edges)$ be a program and $\loc \in \locs$ be a location for which we want to compute a bound.
Our analysis consists of four main steps:

\smallskip

\noindent \fbox{\begin{minipage}{12cm}
%\textbf{Input:} program $\prog = (\locs,\edges)$, location $\loc \in \locs$\\

1. Extract a set of norms $\norms$ using heuristics\hfill(Section~\ref{sec:heuristics})\\
2. Compute global invariants by standard abstract domains \hfill \\
3. Compute $\transinv = \TransSys(\prog,\loc)$ \hfill (Section~\ref{sec:abstraction})\\
4. Compute $\bound = \ComputeBound(\Contextualize(\transinv))$ \hfill (Section~\ref{sec:bound-computation})
%\textbf{Output:} bound $\bound$ for the number of visits to $\loc$
\end{minipage}}

\smallskip

\noindent In Step 1 we extract a set of norms $\norms$ using the heuristics described in Section~\ref{sec:heuristics}. The abstraction function $\alpha$ that we use in Steps 3 and 4 is parameterized by the set of norms $\norms$.
In Step 2 we compute global invariants by standard abstract domains such as interval, octagon or polyhedra.
As this step is standard, we do not discuss it in this paper.
In Step 3 we compute a transition system $\transinv = \TransSys(\prog,\loc)$ for $\prog|_\loc$ by Algorithm~\ref{alg:transitionSystem}.
%, which enumerates all cycle-free paths from $\loc$ back to $\loc$ and derives a disjunctive transition system $\transinv$ from these paths and the summaries of the inner loops using pathwise analysis.
In Step 4 we compute a bound $\bound = \mathtt{Bound}(\mathtt{Contextualize}(\transinv))$ for the number of visits to $\loc$, where we first use the program transformation contextualization of Definition~\ref{def:contextualization} to transform $\transinv$ into a program from which we then compute a bound $\bound$ by Algorithm~\ref{alg:computeBound}.

%The key insight of our method is to use SCA observes the monotonic changes of norms.
%-> powerful termination / bound analysis as fixed points can be effectively computed
%-> expressiveness limited, thus preprocessing helpful to increase precision

%In order to handle loop we need some abstraction which allow to compute fixed points for establishing inductive invariants.

%In steps 3 and there are the following key choices: program transformations for problem simplification, abstraction, fixed point computation for reasoning about loops

\vspace{-0.4cm}

\begin{algorithm}
%\vspace{-0.5cm}
\SetKwInput{Procedure}{Procedure}
\Procedure{$\TransSys(\prog, \loc)$}
%\Procedure{$test$}
\KwIn{a program $\prog = (\locs,\edges)$, a location $\loc \in \locs$}
\KwOut{a transition system for $\prog|_\loc$}
\SetKwInput{Global}{Global}
%\SetKwData{Summary}{summary}
\Global{array $\Summary$ for storing transition invariants
%, initialized by $\Summary[*] := \{Id\}$
}
\vspace{1mm}
\SetKwFunction{ImmediateNestedLoops}{immediateNestedLoops}
%\SetKwFunction{Header}{header}
%\SetKwFunction{IsHeader}{isHeader}
%\SetKwFunction{ITE}{ITE}

\SetKwFunction{Hull}{Hull}
\SetKwFunction{Paths}{Paths}
\SetKwFunction{Unroll}{Unroll}
\ForEach{$(\looop,\header) \in NestedLoops(\prog,\loc)$}{
   $\transinv := \TransSys(\looop,\header)$\;
%   $(\mathit{next},\mathit{exit}) := \Unroll(\transinv)$\;
%   $\closure := \gamma(\alpha(next)^*)$\;
   $\closure := \gamma(\alpha(\transinv)^*)$\;
%   $\Summary[\header] := \closure \circ exit$\;
   $\Summary[\header] := \closure$\;
}
\ForEach{cycle-free path $\paath = \loc \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \loc_2 \cdots \loc_k \xrightarrow{\trn_k} \loc \in \mathtt{paths}(\prog,\loc)$}{
%  \For{$i := 1$ \KwTo $k-1$}{
%    \lIf{$\IsHeader(\loc_i)$}{$\transinv_i := \Summary[\loc_i]$\;}
%    \lElse{$\transinv_i := \{Id\}$\;}
%  }
%  $\transinv := \transinv \cup (\{\trn_0\} \circ \transinv_1 \circ \{\trn_1\} \circ \transinv_2 \circ \{\trn_2\} \circ \cdots \circ \transinv_{k-1} \circ \{\trn_{k-1}\})$\;
%  $\transinv_\loc := \transinv_\loc \cup \{\trn_0\} \circ \Summary[\loc_1] \circ \{\trn_1\} \circ \Summary[\loc_2] \circ$\\
%  $\quad \quad \quad \quad \quad \{\trn_2\} \circ \cdots \circ \Summary[\loc_k] \circ \{\trn_k\}$\;
  $\transinv_\paath := \{\trn_0\} \circ \ITE(\IsHeader(\loc_1),\Summary[\loc_1], \{Id\}) \circ \{\trn_1\} \circ$\\
  $\quad \quad \quad \quad \quad \ \ \ \ITE(\IsHeader(\loc_2),\Summary[\loc_2], \{Id\}) \circ \{\trn_2\} \circ \cdots \circ$\\
  $\quad \quad \quad \quad \quad \ \ \ \ITE(\IsHeader(\loc_k),\Summary[\loc_k], \{Id\}) \circ \{\trn_k\}$\;
}
\Return $\bigcup_{\text{cycle-free path } \paath \in \mathtt{paths}(\prog,\loc)} \transinv_\paath$\;
\caption{$\TransSys(\prog,\loc)$ computes a transition system for $\prog|_\loc$}
\label{alg:transitionSystem}
%\vspace{-0.75cm}
\end{algorithm} 

==> include/app_examples.tex <==
\section{Examples}

\subsection{Example application of Algorithm~\ref{alg:transitionSystem}}
\label{app:alg1example}

%\noindent{\bf Example \ref{ex:abstraction}}
Let $\prog$ be the program of Example~\ref{ex:abstraction}.
We want to compute the transition system for $\prog|_{\loc_1}$ and hence call $\TransSys(\prog,\loc_1)$.
%We show how Algorithm~\ref{alg:transitionSystem} computes $\TransSys(\prog,\loc_1)$, where $\prog$ is the program of Example~\ref{ex:abstraction}.
In the first {\tt foreach}-loop Algorithm~\ref{alg:transitionSystem} calls itself recursively on the nested loop $\looop = (\{\loc_2\},\{\loc_2 \xrightarrow{\trn_2} \loc_2\})$ with header $\loc_2$.
In the recursive call Algorithm~\ref{alg:transitionSystem} skips the first {\tt foreach}-loop because $(\looop,\loc_2)$ does not have nested loops.
The second {\tt foreach}-loop iterates over all cycle-free paths of $\mathtt{paths}(\looop,\loc_2)$.
There is only one such a path $\paath = \loc_2 \xrightarrow{\trn_2} \loc_2$.
Algorithm~\ref{alg:transitionSystem} computes $\transinv_\paath = \{i < n \wedge i^\prime = i + 1 \wedge j^\prime = j + 1 \wedge n^\prime = n \}$ and returns $\transinv_\paath$ as the transition system $\TransSys(\looop,\loc_2)$.
After the return of the recursive call $\transinv = \TransSys(\looop,\loc_2)$ Algorithm~\ref{alg:transitionSystem} size-change abstracts $\transinv$ by $\alpha(\transinv) = \{n - i > 0 \wedge n^\prime - i^\prime < n - i  \wedge j < j'\}$, computes the reflexive transitive hull in the abstract $\alpha(\transinv)^* = \{{n^\prime - i^\prime = n - i} \wedge {j^\prime = j}, {n - i > 0} \wedge {n^\prime - i^\prime < n - i} \wedge {j^\prime > j}\}$ and stores $\gamma(\alpha(\transinv)^*)$ in $\Summary[\loc_2]$.
As there is no other nested loop the first {\tt foreach}-loop is finished.
The second {\tt foreach}-loop iterates over all cycle-free paths of $\mathtt{paths}(\prog,\loc_1)$.
There are two such paths $\paath_1,\paath_2$ as explained in Section~\ref{subsec:example-abstraction}.
Algorithm~\ref{alg:transitionSystem} computes
$\transinv_{\paath_1} = \{\trn_1\} \circ \Summary[\loc_2] \circ \{\trn_3\} =
\{n - i > 0 \wedge i_1 = i + 1 \wedge j_1 = 0 \wedge  n^\prime - i^\prime = n - i \wedge j^\prime = j_1 \wedge j^\prime > 0,  i_1 = i + 1 \wedge j_1 = 0 \wedge n - i_1 > 0 \wedge n^\prime - i^\prime < n - i \wedge j^\prime > j_1 \wedge j^\prime > 0\} =
\{false, n - i - 1 > 0 \wedge {n^\prime - i^\prime < n - i} \wedge j^\prime > 0\}$,
$\transinv_{\paath_2} = \{\trn_1\} \circ \Summary[\loc_2] \circ \{\trn_4\}=
\{n - i > 0 \wedge i_1 = i + 1 \wedge j_1 = 0 \wedge n^\prime - i^\prime = n - i_1  \wedge j^\prime = j_1 \wedge j^\prime = 0, i_1 = i + 1 \wedge j_1 = 0 \wedge n - i_1 > 0  \wedge n^\prime - i^\prime > n - i_1 \wedge j^\prime > j_1 \wedge j^\prime = 0\} =
\{n - i > 0 \wedge n^\prime - i^\prime = n - i - 1 \wedge j^\prime = 0, false\}$ and returns $\transinv_{\paath_1} \cup \transinv_{\paath_2} = \{n - i - 1 > 0 \wedge n^\prime - i^\prime < n - i \wedge j^\prime > 0,n - i > 0 \wedge n^\prime - i^\prime = n - i - 1 \wedge j^\prime = 0\}$ as transition system for $\prog|_{\loc_1}$.

\subsection{Example application of Algorithm~\ref{alg:computeBound}}
\label{app_alg2examples}

%\noindent{\bf Example \ref{ex:state-machine}}
The CFG in Figure~\ref{fig:cfg1} has 5 SCCs: ($\loc_1$), ($\loc_2$), ($\loc_3$), ($\loc_4$), ($\loc_5$, $\loc_6$).
Algorithm~\ref{alg:computeBoundSCC} computes the following bounds on these SCCs: $\bound_{\loc_1} = \max(255 - s, 0)$, $\bound_{\loc_2} = \max(s, 0)$, $\bound_{\loc_3} = 1$, $\bound_{\loc_4} = 1$, $\bound_{\loc_5, \loc_6} = l = \log{c}$.
Algorithm~\ref{alg:computeBound} composes these bounds as follows:
$\max(u(\bound_{\loc_1}), u(\bound_{\loc_2})) + \max(u(\bound_{\loc_3}), u(\bound_{\loc_4})) + u(\bound_{\loc_5, \loc_6})$, where $u$ denotes an upper bound on the value of the given expression computed by an invariant analysis.
Assuming that the invariant analysis provides $u(\bound_{\loc_1}) = 255$, $u(\bound_{\loc_2}) = s$, $u(\bound_{\loc_3}) = 1$, $u(\bound_{\loc_4}) = 1$ and $u(\bound_{\loc_5, \loc_6}) = 2$, we obtain the precise bound $\max(255, s) + 3$.
%$u(\max(\bound_{\loc_1}, \bound_{\loc_2})) = \max(255, s)$, $u(\max(\bound_{\loc_3}, \bound_{\loc_4})) = 1$, $u(\bound_{\loc_5, \loc_6}) = 2$, we obtain the precise bound $\max(255, s) + 3$.\todo{M: nach alg 2 muss es heissen: $\max(u(\cdots),u(\cdots))$ anstatt $u(\max(\cdots))$.}
%, which differs only by one from the exact bound $\max(255, start) + 2$, which is due to contextualization.


\subsection{Flagship Example of ~\cite{conf/pldi/GulwaniJK09}}
\label{subsec:flagship-example-appendix}

In this subsection we apply our analysis to the flagship example of a recent publication~\cite{conf/pldi/GulwaniJK09} on the bound problem (Example~\ref{ex:cyclic} below).
On this example the authors of~\cite{conf/pldi/GulwaniJK09} motivate control-flow refinement for bound analysis.
Their algorithm relies on a sophisticated interplay between control-flow refinement and abstract interpretation.
We show that our simpler technique can also handle the example.
%Contextualization can also handle the example,% as we explain in the following,
%what shows the strength of our simpler technique.

\begin{example}
\label{ex:cyclic}
\begin{verbatim}
void cyclic(int id, int maxId) {
assume(0 <= id <= maxId);
int tmp := id+1;
while(tmp !=id && nondet()){
    if (tmp <= maxId) tmp := tmp + 1;
    else tmp := 0; } }
\end{verbatim}
\end{example}

We assume an invariant analysis (e.g. octagon analysis) provides the invariant $0 \le \mathit{id} \le \mathit{maxid} \wedge \mathit{tmp} \ge 0$ at the header of the $\mathtt{while}$-loop.
%
The $\mathtt{while}$-loop has four paths because we consider the inequality {\tt tmp != id} as the disjunction $\mathit{tmp} < \mathit{id} \vee \mathit{tmp} > \mathit{id}$.
Algorithm~\ref{alg:transitionSystem} gives us the transition system $\transinv = \{\trn_1,\trn_2,\trn_3\}$ (there is no fourth transition because $0 \le \mathit{id} \le \mathit{maxid} \wedge \mathit{tmp} < \mathit{id} \wedge \mathit{tmp} > \mathit{maxid}$ is unsatisfiable), where

\smallskip

{\small
\noindent $\trn_1 \equiv {{0 \le id \le \mathit{maxid}} \wedge \mathit{id} < \mathit{tmp} \le \mathit{maxid} \wedge \mathit{tmp}^\prime = \mathit{tmp} + 1}$,\\
$\trn_2 \equiv {{0 \le \mathit{id} \le \mathit{maxid}} \wedge \mathit{tmp} > \mathit{maxid}  \wedge \mathit{tmp}^\prime = 0}$,\\
$\trn_3 \equiv {{0 \le \mathit{id} \le \mathit{maxid}} \wedge 0 \le \mathit{tmp} < \mathit{id} \wedge \mathit{tmp}^\prime = \mathit{tmp} + 1}$.
}

\smallskip

\begin{figure}
\input{Examples/example23CFG}
\caption{Contextualization of Example \ref{ex:cyclic}
%(left) and \ref{ex:kroening} (right) after contextualization.
\label{fig:cfgbound}
}
\end{figure}

Contextualization gives us the CFG depicted in Figure~\ref{fig:cfgbound}, which precisely reflects the different phases of the loop.
%Algorithm~\ref{alg:computeBound} (stated in the next subsection) exploits the CFG structure in order to compute the bound $\mathit{maxId} + 1$ (cf. Subsection~\ref{app_alg2examples})

The control flow graph given in Figure~\ref{fig:cfgbound} has 3 SCCs: ($\loc_1$), ($\loc_2$), ($\loc_3$).
Algorithm~\ref{alg:computeBoundSCC} computes the following bounds on these SCCs:
$\bound_{\loc_1} = \max(maxId - tmp, 0)$, $\bound_{\loc_2} = 1$ and $\bound_{\loc_3} = \max(id - tmp, 0)$.
Algorithm~\ref{alg:computeBound} composes these bounds as follows:
$u(\bound_{\loc_1}) + u(\bound_{\loc_2}) + u(\bound_{\loc_3})$, where $u$ denotes an upper bound on the value of the given expression.
Assuming that the invariant analysis provides $u(\bound_{\loc_1}) = maxId - id$, $u(\bound_{\loc_2}) = 1$, $u(\bound_{\loc_3}) = id$, we obtain the precise bound $maxId + 1$. 

==> include/blockpath.tex <==

\section{Comparison between Blockwise and Pathwise SCA Analysis}
\label{sec:blockpath}

Classical papers on termination analysis with SCA~\cite{conf/popl/LeeJB01,journals/acta/Ben-Amram09} do not discuss how one can obtain abstract programs.
However, these papers assume that abstract programs are given as CFGs whose edges are labeled by SCRs.
Therefore it is fair to say that classical SCA uses blockwise analysis.
We sketch how this abstraction strategy differs from our approach:
Classical SCA abstracts program in one step, and then analyzes the abstracted programs by a single transitive hull computation.
%pathwise abstraction with SCA = path enumerating + unrolling,
%We correspond to the difficulty by path enumerating and unrolling.
In contrast, our pathwise analysis abstracts programs in multiple steps and computes transitive hulls at multiple times during the analysis.
Our approach is a generalization of classical SCA and strictly more precise.
%We recursively compute transition systems for inner loops, abstract these summaries to SCR sets, compute transitive hulls of the SCR sets, and use the concretizations of the abstract transitive hulls for enumerating paths.

We illustrate the difference between our pathwise analysis and classical SCA in the following.
Let $\prog$ be the program in Example~\ref{ex:abstraction}.
As described in Section~\ref{app:alg1example} we obtain the transition system $\TransSys(\prog,\loc_1) = \{n - i - 1 > 0  \wedge n^\prime - i^\prime < n - i \wedge j^\prime > 0, n - i > 0  \wedge  n^\prime - i^\prime = n - i - 1 \wedge j^\prime = 0\}$ for $\prog|_{\loc_1}$ by pathwise analysis.
Note that $\TransSys(\prog,\loc_1)$ establishes that the variable $i$ increases at every loop iteration and that $i < n$ is an invariant at $\loc_1$.
$\TransSys(\prog,\loc_1)$ is precise enough so that our Algorithm~\ref{alg:computeBound} can further size-change abstract it and compute a bound from the abstraction.

The blockwise analysis in classical SCA begins with abstracting $\prog$.
Because of the inner loop at location $\loc_2$ of program $\prog$, each transition $\trn_1,\trn_2,\trn_3,\trn_4$ constitutes a program block and needs to be abstracted separately.
We get the SCRs $\alpha(\trn_1) = n - i > 0  \wedge n^\prime - i^\prime < n - i \wedge j^\prime \ge 0, \alpha(\trn_2) = n - i > 0  \wedge n^\prime - i^\prime < n - i \wedge j < j^\prime, \alpha(\trn_3) = j > 0 \wedge n^\prime - i^\prime > n - i, \alpha(\trn_4) = j \le 0 \wedge  n^\prime - i^\prime = n - i$.
The termination analysis with classical SCA computes the transitive hull of these SCRs along the control flow edges of program $\prog$.
In particular classical SCA computes the SCR
$\alpha(\trn_1) \circ \alpha(\trn_2) \circ \alpha(\trn_3) = n - i > 0 \wedge j^\prime > 0$ for the path $\loc_1 \xrightarrow{\trn_1} \loc_2 \xrightarrow{\trn_2} \loc_2 \xrightarrow{\trn_3} \loc_1$.
Note that classical SCA cannot establish that $n-i$ increases every time this path is taken (the concatenation of  $n^\prime - i^\prime < n - i$ and $n^\prime - i^\prime > n - i$ in $\alpha(\trn_2)$ and $\alpha(\trn_3)$ loses all information on $n-i$) and therefore cannot prove the termination of $\prog$.



==> include/bound.tex <==
\svnid{$Id$}
%\vspace{-0.3cm}
\section{Bound Computation}
\label{sec:bound-computation}
%\vspace{-0.2cm}
Our bound computation consists of two steps. Step 1 is the program transformation contextualization which transforms a transition system into a program. Step 2 is the bound algorithm which computes bounds from programs.
\vspace{-0.2cm}
\subsection{Contextualization}
\label{subsec:contextualization}
\vspace{-0.1cm}
Contextualization is a program transformation by Manolios and Vroon~\cite{conf/cav/ManoliosV06}, who report on an impressive precision of their SCA-based termination analysis of functional programs. Note that we do not use their terminology (e.g. ``calling context graphs'') in this paper. Our contribution lies in adopting contextualization to imperative programs and in recognizing its relevance for bound analysis.

%, such that every location stores the context of which transition is to be executed next and such that there is an edge between two locations only if the transitions of the locations can be executed one after another.

\begin{definition}[Contextualization]
\label{def:contextualization}
  Let $\transinv$ be a transition set.
  The \emph{contextualization} of $\transinv$ is the program $\prog = (\transinv,\edges)$, where $\edges = \{ \trn \xrightarrow{\trn} \trn^\prime \mid \trn,\trn^\prime \in \transinv \text{ and } \trn \circ \trn^\prime \neq \emptyset \}$.
\end{definition}

The contextualization of a transition system is a program in which every location determines which transition is executed next;
the program has an edge between two locations only if the transitions of the locations can be executed one after another.

Contextualization restricts the order in which the transitions of the transition system can be executed.
Thus, contextualization encodes information that could otherwise be deduced
from the pre- and postconditions of transitions directly into the CFG.
Since pathwise analysis contracts whole loop paths into single transitions, contextualization is particularly important after pathwise analysis:
our subsequent bound algorithm does not need to compute the pre- and postcondition of the contracted loop paths but only needs to exploit the structure of the CFGs for determining in which order the loop paths can be executed.

%Contextualization shows its strength in Example~\ref{ex:contextualize1}.
%
%\begin{example}
%\label{ex:contextualize1}
%\begin{verbatim}
%void main ( ) {
%int x;
%while (x != 0){
%  if (x > 0) x = x - 1;
%  else if (x < 0) x = x + 1;
%} }
%\end{verbatim}
%\end{example}
%
%Contextualization can be generalized to $k$-contextualization.
%
%\begin{definition}[$k$-Contextualization]
%  Let $\transinv$ be a transition set.
%  The $k$-\emph{contextualization} of $\transinv$ is the program $\prog = (\{(\trn_1,\ldots,\trn_k) \mid \trn_1,\ldots,\trn_k \in \transinv\},\edges)$, where $\edges = \{ (\trn_1,\ldots,\trn_k) \xrightarrow{\trn_1} (\trn_2,\ldots,\trn_{k+1}) \mid \trn_1,\ldots,\trn_{k+1} \in \transinv \text{ and } \trn_1 \circ \cdots \circ \trn_k \neq \emptyset \}$.
%  \todo{problem that $\transinv^k$ is already used for $k$-fold concatenation}
%\end{definition}
%
%$k$-Contextualization is more precise for increasing values of $k$.
%An example for this fact are loops that can only be repeated $k-1$ times.
%Another example is given by Example~\ref{ex:contextualize2} - an extension of Example~\ref{ex:contextualize1}.
%
%\begin{example}
%\label{ex:contextualize2}
%\begin{verbatim}
%void main ( ) {
%int x;
%int flag = 0;
%while (x != 0){
%  if (flag = 0){
%    if (x > 0) x = x - 1;
%    else if (x < 0) x = x + 1;
%    flag = k; }
%  else if (flag = k)
%    flag = k-1;
%  else if (flag = k-1)
%    flag = k-2;
%  ...
%  else if (flag = 1)
%    flag = 0;
%} }
%\end{verbatim}
%\end{example}
%
%Example~\ref{ex:contextualization-not-sufficient} can not be handled by $k$-contextualization combined with SCA.
%The path that decreases $y$ can be repeated arbitrarily often.
%Therefore no $k$-window can track the information that either $x > 0$ or $x < 0$ is invariant.
%We see from Example~\ref{ex:contextualization-not-sufficient} that $k$-contextualization does not help when inductive invariants are needed.
%
%\begin{example}
%\label{ex:contextualization-not-sufficient}
%\begin{verbatim}
%void main ( ) {
%int x,y;
%while (x != 0 && y > 0){
%  if (nondet()){
%    if (x > 0) x = x - 1;
%    else if (x < 0) x = x + 1; }
%  else
%    y--;
%} }
%\end{verbatim}
%\end{example}

\begin{figure}
\vspace{-0.5cm}
\begin{tabular}{llc}
\begin{minipage}[c]{4.5cm}

\begin{example}
\label{ex:no-inv-needed}
\begin{verbatim}

void main (int x, int b){
while (0 < x < 255){
  if (b) x = x + 1;
  else x = x - 1; } }
\end{verbatim}
\end{example}

\end{minipage}

&

\begin{minipage}[c]{6cm}
{\small
\noindent $\trn_1 \equiv {{0 < x < 255} \wedge b \wedge x^\prime = x + 1 \wedge b^\prime}$\\
$\trn_2 \equiv {{0 < x < 255} \wedge \neg b \wedge x^\prime = x-1 \wedge \neg b^\prime}$
}
\end{minipage}

&

\begin{minipage}[c]{3cm}

\begin{tikzpicture}[scale=0.5, node distance = 1cm, auto,label distance=2mm]
\node         (f1)  {$\loc_1$};
\node         (f2) [right of=f1]  {$\loc_2$};

\path (f1) edge [loop below] node {$\trn_1$} (f1)
(f2) edge [loop below] node {$\trn_2$} (f2);
\end{tikzpicture}

\end{minipage}
\end{tabular}
\caption{Example~\ref{ex:no-inv-needed} with its transition relations and CFG obtained from contextualization.\label{fig:cfg-no-inv-needed}}
\vspace{-0.5cm}
\end{figure}

We illustrate contextualization on Example~\ref{ex:no-inv-needed}.
The program has two paths, and gives rise to the transition system $\transinv = \{\trn_1,\trn_2\}$.
Keeping track of the boolean variable $b$ is important for bound analysis:
Without reference to $b$ not even the termination of $\mathtt{main}$ can be proven.
In Figure~\ref{fig:cfg-no-inv-needed} (right) we show the contextualization of $\transinv$.
Note that contextualization has encoded information about the variable $b$ into the CFG in such a way that we do not need to keep track of the variable $b$ anymore.
Thus, contextualization releases us from taking the precondition $b$ resp. $\neg b$ and the postcondition $b^\prime$ resp. $\neg b^\prime$ into account for bound analysis.

%It is a general fact that contextualization encodes information that can be deduced from the pre- and postconditions of transitions into the CFG.
%This achieves a separation of control and transition invariants
%as our subsequent bound algorithm is released from taking these conditions into account and only needs to exploit the structure of the CFG.

At the beginning we gave an application of contextualization on the sophisticated loop in Example~\ref{ex:state-machine}, where contextualization uncovers the control structure of the finite state machine encoded into the loop.
\final{An application of contextualization to the flagship example of a recent publication~\cite{conf/pldi/GulwaniJK09} can be found in the extended version of this paper.}
\full{An application of contextualization to the flagship example of a recent publication~\cite{conf/pldi/GulwaniJK09} can be found in Section~\ref{subsec:flagship-example-appendix} of the appendix.}

Note that in our definition of contextualization we only consider the consistency of two consecutive transitions.
It would also have been possible to consider three or more consecutive transitions.
This would result in increased precision.
However, we found two transitions to be sufficient in practice.

\noindent\emph{Implementation.}
We implement contextualization by encoding the concatenation $\trn_1 \circ \trn_2$ of two transitions $\trn_1,\trn_2$ into a logical formula and asking an SMT solver whether this formula is satisfiable.
Note that such a check is very simple to implement in comparison to the explicit computation of pre- and postconditions. %which is a difficult problem in general.
\vspace{-0.6cm}

%\todo{The further explanations could probably be left out}
%The bound algorithm uses only the following monotonicity constraints obtained from size-change abstracting the transitions:
%$\mathit{maxId} - \mathit{tmp} \ge \mathit{maxId} - \mathit{id}, \mathit{maxId} - \mathit{tmp} > (\mathit{maxId} - \mathit{tmp})^\prime \in \alpha(\trn_1)$,
%none from $\alpha(\trn_2)$, $\mathit{id} - \mathit{tmp} \ge 0, \mathit{id}- \mathit{tmp} > (\mathit{id} - \mathit{tmp})^\prime \in \alpha(\trn_3)$.
%Note that do not have to use the pre- and postconditions inferable from the transitions relations which would be necessary to distinguish the different loop phases.
%In particular that we do not have to use the postcondition $\mathit{tmp}^\prime \le id$ of the third condition.
%Extracting the predicate $\mathit{tmp}^\prime \le id$ is normally a difficult step in a static analysis because it does not appear in the program code.
%We only use the minimal number of predicates needed for bounding the number of iterations of the particular loop phases.

%Note that SCA is strong enough to prove termination on its own, but $\scr_3$ need to contain the predicate $tmp ^\prime <= id$
%\begin{itemize}
%\item $\scr_1 \equiv 0 \le id \le maxid \wedge id < tmp <= maxid \wedge tmp^\prime > tmp$
%\item $\scr_2 \equiv 0 \le id \le maxid \wedge tmp > maxid  \wedge tmp^\prime = 0$
%\item $\scr_3 \equiv 0 \le id \le maxid \wedge 0 \le tmp < id \wedge tmp^\prime > tmp \wedge tmp ^\prime <= id$
%\end{itemize}

%Kroening et al.~\cite{conf/cav/KroeningSTW10} use the following program to present their termination analysis.
%
%\begin{example}
%\label{ex:kroening}
%\begin{verbatim}
%void main ( ) {
%int x;
%int debug = 0;
%while (x < 255)
%if (x%2 != 0) x--;
%else x+=2;
%if (debug != 0) x=0;}
%\end{verbatim}
%\end{example}
%
%We require a lightweight invariant analysis such as the interval analysis to compute the invariant $\mathit{debug} = 0$ at the loop header.
%
%The loop has four program paths, what results into two transitions when taking $\mathit{debug} = 0$ into account:
%
%\smallskip
%
%{\small
%\noindent $\trn_1 \equiv {{x < 255} \wedge {{x \mod 2} \neq 0} \wedge {x^\prime = {x - 1}}}$\\
%$\trn_2 \equiv {{x < 255} \wedge {{x \mod 2} = 0} \wedge {x^\prime = {x + 2}}}$
%}
%
%\smallskip
%
%SCA gives us the following size-change relations:
%
%\smallskip
%
%{\small
%\noindent $\scr_1 \equiv x < 255 \wedge x^\prime < x$\\
%$\scr_2 \equiv x < 255 \wedge x^\prime > x$
%}
%
%\smallskip
%
%Note that $\scr_1$ is not well-founded and thus a direct application of SCA termination or bound analysis fails.
%Contextualization however results in the CFG depicted in Figure~\ref{fig:cfgbound}(right).
%
%However, contextualization gives us the following CFG:
%\begin{displaymath}
%\trn_1 \xrightarrow{\scr_1} \trn_2, \trn_2 \xrightarrow{\scr_2} \trn_2
%\end{displaymath}
%\TODO{draw CFG}
%
%The CFG shows us that $\trn_1$ can be executed only once, and thus we do not have to take $\scr_1$ for termination / bound analysis into account.


%
%However by unrolling $\trn_1 | \trn_2$ to $\trn_1\trn_1 | \trn_1\trn_2 | \trn_2\trn_1 | \trn_2\trn_2$ we obtain the program:
%\begin{itemize}
%\item $\trn_1 \circ \trn_2 \equiv x < 255 \wedge x \mod 2 \neq 0 \wedge x^\prime = x + 1$
%\item $\trn_2 \circ \trn_1 \equiv x < 255 \wedge x \mod 2 = 0 \wedge x^\prime = x + 1$
%\end{itemize}
%Note that $\trn_1\trn_1$ and $\trn_2\trn_2$ have been omitted because they are not satisfiable, which can be proven by an SMT solver capable of integer reasoning.
%
%Abstracting the unrolled program results in an SCS that can prove termination:
%\begin{itemize}
%\item $\scr{12} \equiv x < 255 \wedge x^\prime > x$
%\item $\scrs{21} \equiv x < 255 \wedge x^\prime > x$
%\end{itemize}
%
%The SCS is already terminating as $255 - x$ is a ranking function on both transitions.
\begin{algorithm}
\SetKwInput{Procedure}{Procedure}
\Procedure{{\tt Bound}$(\prog)$}
\KwIn{a program $\prog = (\locs,\edges)$}
\KwOut{a bound $\bound$ on the length of the traces of $\prog$}
\SetKwFunction{ComputeSCCs}{computeSCCs}
$\SCCs := \ComputeSCCs($\prog$)$; $\bound := 0$\;
\While{$\SCCs \neq \emptyset$}{
  $\SCCsOnLevel := \emptyset $\;
  \ForAll{$\SCC \in \SCCs$ s.t. no $\SCC^\prime \in \SCCs$ can reach $\SCC$}{
    $r := \ComputeBoundSCC(\SCC)$\;
    Let $r \le \bound_\SCC$ be a global invariant\;
    $\SCCsOnLevel := \SCCsOnLevel \cup \{\SCC\}$\;
  }
  $\bound := \bound + \max_{\SCC \in \SCCsOnLevel} \bound_\SCC$\;
  $\SCCs := \SCCs \setminus \SCCsOnLevel$\;

}
\Return $\bound$\;
\caption{{\tt Bound} composes the bounds of the SCCs to an overall bound}
\label{alg:computeBound}
\end{algorithm}

%\vspace{-1.0cm}
\subsection{Bound Algorithm}
\label{subsec:ranking-function-algorithm}

Our bound algorithm reduces the task of bound computation to the computation of local bounds and the composition of these local bounds to an overall bound.
To this end, we exploit the structure of the CFGs obtained from contextualization:
We partition the CFG of programs into its strongly connected components (SCCs) (SCCs are maximal strongly connected subgraphs).
For each SCC, we compute a bound by Algorithm~\ref{alg:computeBoundSCC}, and then compose these bounds to an overall bound by Algorithm~\ref{alg:computeBound}.

%\begin{definition}[Strongly Connected Component (SCC)]
%A {\em strongly connected component} of a directed graph is a maximal strongly connected subgraph. A directed graph is called {\em strongly connected} if there is a path from each vertex in the graph to every other vertex.
%A directed graph is called {\em strongly connected} iff there is a path from each vertex in the graph to every other vertex.
%The {\em strongly connected components} of a directed graph are its maximal strongly connected subgraphs.
%\end{definition}
%\ref{alg:computeBoundSCC} \ref{alg:computeBound}

\nop{Let $\prog$ be a program that consists of the two SCCs $\SCC_1$ and $\SCC_2$ with the respective bounds $\bound_{\SCC_1}$ and $\bound_{\SCC_2}$.
$\max(\bound_{\SCC_1},\bound_{\SCC_2})$ is an upper bound for $\prog$, if every execution of $\prog$ either stays in $\SCC_1$ or $\SCC_2$.}


\noindent Algorithm~\ref{alg:computeBound} arranges the SCCs of the CFG into levels:
The first level consists of the SCCs that do not have incoming edges,
the second level consists of the SCCs that can be reached from the first level, etc.
For each level, Algorithm~\ref{alg:computeBound} calls Algorithm~\ref{alg:computeBoundSCC} to compute bounds for the SCCs of this level.
Let $\SCC$ be an SCC of some level and let $r := \ComputeBoundSCC(\SCC)$ be the bound returned by Algorithm~\ref{alg:computeBoundSCC} on $\SCC$.
$r$ is a (local) bound of $\SCC$ that may contain variables of $\prog$ that are changed during the execution of $\prog$.
%These bounds may contain program variables, whose initial values may depend on the SCCs of the earlier level.
Algorithm~\ref{alg:computeBound} uses global invariants (e.g. interval, octagon or polyhedra) in order to obtain a bound $\bound_\SCC$ on $r$ in terms of the initial values of $\prog$.
The SCCs of one level are collected in the set $\SCCsOnLevel$.
For each level, Algorithm~\ref{alg:computeBound} composes the bounds $\bound_\SCC$ of all SCCs $\SCC \in \SCCsOnLevel$ to a maximum expression.
Algorithm~\ref{alg:computeBound} sums up the bounds of all levels for obtaining an overall bound.

%\vspace{-0.6cm}
\begin{algorithm}
\SetKwInput{Procedure}{Procedure}
\Procedure{{\tt BndSCC}$(\prog)$}
\KwIn{strongly-connected program $\prog = (\locs,\edges)$}
\KwOut{a bound $\bound$ on the length of the traces of $\prog$}
\SetKw{Fail}{fail with}
\lIf{$\edges = \emptyset$}{\Return $1$\;}
$\NonIncr :=  \emptyset$; $\DecrBnded := \emptyset$; $\BndedEdgs := \emptyset$\;
\ForEach{$\norm \in \norms$}{
    \If{${\forall \ {{\loc_1 \xrightarrow{\trn} \loc_2} \in \edges}}\; {{\norm \ge \norm^\prime} \in \alpha(\trn)} $}{
       $\NonIncr := \NonIncr \cup \{\norm\}$\;
    }
}

\ForEach{${\loc_1 \xrightarrow{\trn} \loc_2 \in \edges}$, ${\norm \in \NonIncr}$}{
    \If{$\norm \ge 0, \norm > \norm^\prime \in \alpha(\trn)$}
    {
       $\DecrBnded := \DecrBnded \cup \{\max(\norm, 0)\}$\;
       $\BndedEdgs := \BndedEdgs \cup \{\loc_1 \xrightarrow{\trn} \loc_2\}$\;
    }
}

\lIf{$\BndedEdgs = \emptyset$ }{\Fail ``there is no bound for $\prog$''\;}

$\bound = \ComputeBound((\locs, \edges \setminus \BndedEdgs))$\;

\Return $((\sum \DecrBnded) + 1 ) \cdot \bound$\;
\caption{{\tt BndSCC} computes a bound for a single SCC}
\label{alg:computeBoundSCC}
\end{algorithm}
%\vspace{-0.8cm}

%algorithm \ref{alg:computeBound} and \ref{alg:computeBoundSCC} can be easily adjusted to compute lexicographic ranking functions instead of bounds.

\noindent Algorithm~\ref{alg:computeBoundSCC} computes the bound of a strongly-connected program $\prog$.
First Alg.~\ref{alg:computeBoundSCC} checks if $\prog = (\locs,\edges)$ is trivial, i.e., $\edges = \emptyset$, and returns $1$, if this is the case.
Next Alg.~\ref{alg:computeBoundSCC} collects all norms in the set $\NonIncr$ that either decrease or stay equal on all transitions.
Subsequently Alg.~\ref{alg:computeBoundSCC} checks for every norm $\norm \in \NonIncr$ and transition $\loc_1 \xrightarrow{\trn} \loc_2 \in \edges$, if $\norm$ is bounded from below by zero and decreases on $\trn$.
If this is the case, Alg.~\ref{alg:computeBoundSCC} adds $\max(\norm,0)$ to the set $\DecrBnded$ and $\loc_1 \xrightarrow{\trn} \loc_2$ to $\BndedEdgs$.
Note that the transitions included in the set $\BndedEdgs$ can only be executed as long as their associated norms are greater than zero.
Every transition in $\BndedEdgs$ decreases an expression in $\DecrBnded$ when it is taken.
As the expressions in $\DecrBnded$ are never increased,
the sum of all expressions in $\DecrBnded$ is a bound on how often the transitions in $\BndedEdgs$ can be taken.
If $\DecrBnded$ is empty, Alg.~\ref{alg:computeBound} fails, because the absence of infinite cycles could not be proven.
Otherwise we recursively call Alg.~\ref{alg:computeBound} on $(\locs, \edges \setminus \BndedEdgs)$ for a bound $\bound$ on this subgraph.
The subgraph can at most be entered as often as the transitions in $\BndedEdgs$ can be taken plus one (when it is entered first).
Thus, $((\sum \DecrBnded) + 1 ) \cdot \bound$ is an upper bound for $\prog$.

\emph{Role of SCA in our Bound Analysis.}
Our bound analysis uses the size-change abstractions of transitions to determine how a norm $n$ changes according to $n \geq n'$, $n > n'$, $n \geq 0$ in Alg.~\ref{alg:computeBoundSCC}.
We plan to incorporate inequalities between different norms (like $n \geq m'$) in future work to make our analysis more precise.
%Thus, our bound analysis is a simple greedy algorithm, which does not exploit the full power of SCA.
%However, we obtain an efficient algorithm in this way, which is sufficient to handle many programs occurring in practice, when used in combination with the earlier described program transformations.
%\todo{paragraph vague and unclear. why greedy ?}

\emph{Termination analysis.}
If in Algorithm~\ref{alg:computeBound} the global invariant analysis cannot infer an upper bound on some local bound, the algorithm fails to compute a bound, but we can still compute a lexicographic ranking function, which is sufficient to prove termination.
The respective adjustment of our algorithm is straightforward.

% it is possible to introduce a new variable as an upper bound, report this to the user and continue with the analysis. We mention that this approach is sufficient to prove program termination, but the focus of this paper is bounds analysis.\todo{H: check if correct}

%We leave out the detail here for lack of space as our main interest is bound analysis.

%Multiplying the resulting bound with the sum ... + 1. We have to add 1 because we could enter the subgraph directly.%Since the symoblic bound returned by that recursive call is in terms of each time we enter this subgraph, we have to multiply it with the bound.....%is resetted on some transition(s) of $\scs$, we have to compute an upper bound on that symbolic bound before building the product.

%Suming up the bounds for all bounded transitions results in a valid upper bound on the length of any execution based on a path that contains any of the bounded transitions infinitely often.

%Since the value of the symbolic bound that results from the recursive call is reseted on some transition(s) of $\scs$ (else the recursive call would not have been necessary), we have to compute an upper bound on that symoblic bound that is valid at location $l$  (line xx) before building the product.

%bound the number of times a transition in the SCC can be visited. search for transitions that provably cannot lay on any infinite path through the SCS.
%Afterwards we recursivley continue the computation by calling algorithm \ref{alg:computeBound} on the SCS that results from removing the bounded edges (line xx). Nevertheless the sum is not always the optimal upper bound, often taking the minimum or maximum results in a more precise upper bound, a detailed case distinction is subject to future work.

%In order to compose a preferably precise bound, we only want to sum up the bounds of those SCCs that may be visisted

%Hence we only have to sum up the bounds of SCCs that lay on some path. All other bounds can be summarized by maximum expressions.

%Since the bounds that we compute are symoblic and the values of the variables may be altered in previously visited SCCs,

%The key idea when analyzing $\scs$ to compose the overall bound out of ... This allows us to come up with more precise bounds.
%This allows us to come up with more precise ranking functions / bounds.

%Let $\prog$ be the result of calling Algorithm~\ref{alg:transitionSystem}.
%In this section we explain our approach on computing a bound from $\prog$.

%TODO: define SCCs

%The key idea when analyzing $\prog$ is splitting $\prog$ into its SCCs.
%This allows us to come up with more precise ranking functions / bounds.
%Then the SCCs are analyzed for lexicographic ranking functions.

%We describe how Algorithm~\ref{alg:computeBound} computes the bound for Example~\ref{ex:state-machine} in Section~\ref{app_alg2examples} of the appendix and give a further example in Section~\ref{subsec:flagship-example-appendix}.

\final{We give an example for the application of Algorithm~\ref{alg:computeBound} to Example~\ref{ex:state-machine} and to the flagship example of~\cite{conf/pldi/GulwaniJK09} in the extended version of this paper.}
\full{We give an example for the application of Algorithm~\ref{alg:computeBound} to Example~\ref{ex:state-machine} and to the flagship example of~\cite{conf/pldi/GulwaniJK09} in Section~\ref{app_alg2examples} and \ref{subsec:flagship-example-appendix} of the appendix.}


==> include/comparison.tex <==
\svnid{$Id$}
\section{Detailed Comparison with Related Work}
\label{sec:comparison}


In this section we give a detailed comparison with earlier termination / bound analyses.
%Most notably, these approaches include the {\sc Terminator} tool~\cite{conf/pldi/CookPR06}, and the more recent tools {\sc Loopfrog}~\cite{conf/cav/KroeningSTW10} and {\sc SPEED}~\cite{conf/pldi/GulwaniZ10}.
We show that our bound analysis captures the essential ideas of these approaches in a simpler framework.

%\vspace*{-2mm}
\subsection{Comparison of transition predicate abstraction (TPA) and SCA by Heizmann et al.}
\label{subsec:comparison-TPA-SCA}

In~\cite{conf/sas/HeizmannJP10} Heizmann et al. state that SCA is an instance of the more general technique of TPA~\cite{conf/popl/PodelskiR05}.
In particular they formally show that when a tail-recursive functional program $F$ is translated into an imperative program $\prog$, then an SCA-based termination analysis on $F$ can be mimicked by a TPA-based termination analysis on $\prog$ whose predicates are order relations.

However, \cite{conf/sas/HeizmannJP10} does not
\begin{itemize}
\item deal with general imperative programs, but with programs obtained as translations from functional programs.
    Since functional programs can be size-change abstracted more easily (as explained in our comparison with SCA in Section~\ref{subsec:sca}), this problem setting is much simpler.
\item show how to obtain transition predicates for the independent analysis of imperative programs by TPA.
    It only shows that (as a result of the translation) TPA is more general than SCA.
\item deal with a concrete programming language, and does not deal with  practical issues, or concrete analysis tools.
\item make use of the recent progress of the SCA~\cite{mcs-integers}, where SCA is extended from natural numbers to integers, and deals only with natural numbers.
\end{itemize}

Our paper fills in all these left open gaps.
Moreover, our paper clearly goes beyond the issues discussed in~\cite{conf/sas/HeizmannJP10} by unifying much of the previous work on termination and bound analysis, e.g., see our comparison to {\sc Terminator} in Section~\ref{subsec:terminator}, {\tt SPEED} in Section~\ref{subsec:speed} etc.

While we find it quite intuitive that SCA as well as our more general approach are instances of TPA, we are concerned with a different issue in this paper.
We argue that precisely because of its limited expressiveness SCA is suitable for bound analysis: abstracted programs are simple enough that we can compute bounds for them.
We have shown that imperative programs are amenable to bound analysis by SCA using appropriate program transformations, whereas~\cite{conf/sas/HeizmannJP10} is not concerned with practical issues.

%pathwise analysis and contextualization.

\subsection{Termination Analysis by {\sc Terminator}}
\label{subsec:terminator}

%All of the approaches~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07,conf/lics/PodelskiR04, conf/cav/KroeningSTW10} try to prove that a particular program location can not be visited infinitely often or even try to compute a bound on the number of visits.

The {\sc Terminator} tool~\cite{conf/pldi/CookPR06} is an automatic termination analyzer of imperative programs, which uses TPA~\cite{conf/popl/PodelskiR05} for constructing a Ramsey based termination argument~\cite{conf/lics/PodelskiR04}.

%We compare this analysis to our approach:
Our approach and {\sc Terminator} share the idea of extracting progress measures locally (norms resp. local ranking functions) and composing them for a global analysis (bound resp. termination proof).
Because of its non-constructive nature, the Ramsey based termination argument underlying {\sc Terminator} cannot be used for extracting a global ranking function out of the termination proof.
In contrast, we use SCA for the first time to compose global bounds from bounds on norms.
Earlier work on SCA~\cite{mcs-integers} already has shown how to compute global ranking functions from norms.

In order to apply the Ramsey based termination argument, {\sc Terminator} needs to analyze the transitive hull of programs.
This analysis is the most expensive step in the analysis of {\sc Terminator} and has to be repeated many times.
In contrast, we abstract programs first and then analyze only the transitive hull of the abstract program.
This has huge benefits for the speed of the analysis (further discussed in Section~\ref{subsec:loopfrog}).

TPA can lose precision in every step of the analysis.
In contrast, our pathwise analysis follows the structure of programs and loses precision only at well-defined places.
Our analysis handles paths precisely by conjoining the formulae of the statements along the path (using all theories that can be handled by SMT solvers) and loses precision only when summarizing loops.
However, we handle loops precisely w.r.t. their monotonic behavior of norms:
SCA is closed under taking transitive hulls because of the built-in disjunctiveness of SCA and the transitivity of the order relations, transitive hulls can be computed effectively.

{\sc Terminator} is built on top of a full-fledged software model checker, which implements a complicated CEGAR loop in order to extract predicates and local ranking functions from programs.
%However, it is not reported in~\cite{conf/pldi/CookPR06} what heuristics are used for this extraction.
In contrast, our simple and lightweight static analysis relies only on an SMT solver, our set of transition predicates is fixed in advance (the monotonicity predicates of SCA) and our set of norms is extracted from the program at the beginning of the analysis.
%we describe our heuristics for extracting norms
It is an interesting direction of future work to investigate how to combine these approaches, e.g., by using coarse abstractions for filtering the ``easy cases'' and refining the precision for handling the ``hard cases''.

%Let $\prog = (\locs,\edges)$ be a program, and let $\loc \in \locs$ be a location.
%\cite{conf/popl/BerdineCCDO07,conf/lics/PodelskiR04,conf/cav/KroeningSTW10}
%compute transitive d.wf. forward invariants to prove that $\loc$ cannot be visited infinitely often.
%
%\begin{definition}[Transitive-, Disjunctively Well-founded Transition Set]
%  Let $\transinv$ be a transition set.
%  $\transinv$ is \emph{transitive}, if $\bigcup (\transinv \circ \transinv) \subseteq \bigcup \transinv$.
%  $\transinv$ is \emph{disjunctively well-founded} (d.wf.), if every transition relation $\trn \in \transinv$ is well-founded.
%  $\transinv$ is a \emph{forward invariant} for a transition relation $\trn$, if $\trn^+ \subseteq \bigcup \transinv$.
%\end{definition}
%
%The interest in transition invariants stems from the following theorem.
%
%\begin{theorem}[\cite{conf/lics/PodelskiR04}]
%\label{thm:disjunctive-wellfoundedness-termination}
%  Let $\transinv$ be a transition set that is a transitive d.wf. forward invariant for $\prog|_\loc$.
%  Then $\loc$ cannot be visited infinitely often.
%\end{theorem}
%
%In the following we present transition predicate abstraction (TPA)~\cite{conf/popl/PodelskiR05}, which constitutes the termination analysis underlying {\sc Terminator}~\cite{conf/pldi/CookPR06}.
%
%\begin{definition}[Transition Predicates]
%  We fix a finite set of \emph{transition predicates} (TPs) $\predset$ whose concrete instantiation is not important for this paper.
%  The concretization function $\gamma$ associates a transition relation $\gamma(\pred) \in \trns$ with every TP $\pred \in \predset$.
%  We lift $\gamma$ to sets of TPs by setting $\gamma(\preds) = \bigcap_{\pred \in \preds} \gamma(\pred)$ for a set of TPs $\preds \subseteq \predset$.
%  %A set of TPs $\preds \subseteq \predset$ represents the transition relation given by the intersection of its TPs $\bigcap_{\pred \in \preds} \gamma(\pred)$.
%  %We call $\predtranset = \locs \times \textbf{2}^\predset \times \locs$ the set of \emph{predicate transitions}.
%\end{definition}
%A possible choice is setting $\predset = \mcs$, i.e., taking the monotonicity predicates as TPs.
%As for monotonicity predicates we can define a best abstraction function, because the number of predicates is finite.

%\begin{definition}[Transition Predicate Abstraction]
%  The \emph{TPA function} $\alpha_\predset$ takes a transition relation $\trn$ and returns the TPs that contain $\trn$:
%  \begin{displaymath}
%    \alpha_\predset(\trn) = \{ \pred \in \predset \mid \trn \subseteq \gamma(\pred)\}
%  \end{displaymath}
%
%  We lift the transition predicate abstraction function to programs by setting $\alpha(\prog) = (\locs, \edges_{\predset,\prog})$ with $\edges_{\predset,\prog} = \{\loc_1 \xrightarrow{\alpha_\predset(\trn)} \loc_2 \mid \loc_1 \xrightarrow{\trn} \loc_2 \in \edges\})$.
%  %\edges^\prime)$, where $\edges^\prime =
%
%  The \emph{transition predicate abstraction} is the program $TPA_{\predset,\prog} = (\locs,\edges_{TPA,\predset,\prog})$ where $\edges_{TPA,\predset,\prog}$ is the least set with
%  $\edges_{\predset,\prog} \subseteq \edges_{TPA,\predset,\prog}$ and $\loc_1 \xrightarrow{\alpha_\predset(\preds \circ \trn)} \loc_3 \in \edges_{TPA,\predset,\prog}$ for all $\loc_1 \xrightarrow{\preds } \loc_2 \in \edges_{TPA,\predset,\prog}$, $\loc_2 \xrightarrow{\trn} \loc_3 \in \edges$.
%
%
%  The \emph{transition predicate abstraction} is the program $TPA_{\predset,\prog} = (\locs,\edges_{TPA,\predset,\prog})$ where $\edges_{TPA,\predset,\prog}$ is the least set with
%  $\edges_{\predset,\prog} \subseteq \edges_{TPA,\predset,\prog}$ and $\loc_1 \xrightarrow{\alpha_\predset(\preds \circ \trn)} \loc_3 \in \edges_{TPA,\predset,\prog}$ for all $\loc_1 \xrightarrow{\preds } \loc_2 \in \edges_{TPA,\predset,\prog}$, $\loc_2 \xrightarrow{\trn} \loc_3 \in \edges$.
%
%  The \emph{transition predicate abstraction} $TPA_{\predset,\prog,\loc}$ \emph{w.r.t. location} $\loc$ is the transition set $\transinv_{\predset,\prog,\loc} = \{ \preds \mid (\loc,\preds,\loc) \in \edges_{TPA,\predset,\prog}\}$.
%
%  The \emph{post} operator $\operatorname{post}_{\loc_2 \xrightarrow{\trn} \loc_3,\predset}$, which is parameterized by a transition $\loc_2 \xrightarrow{\trn} \loc_3 \in \edges$, takes a set of predicate transitions $\predtrans$, concatenates every predicate transition that ends in location $\loc_2$ with the transition, and uses the abstraction function to abstract the concatenation of the transition relation and the transition predicate:
%  \begin{displaymath}
%    \operatorname{post}_{\loc_2 \xrightarrow{\trn} \loc_3,\predset}(\predtrans) = \{ (\loc_1, \alpha_\predset(\pred \circ \trn), \loc_3) \mid (\loc_1,\pred,\loc_2) \in \predtrans\}
%  \end{displaymath}
%  We denote the \emph{least fixed point} of the post operator w.r.t. a set of predicate transitions $I$ by $\operatorname{lfp}_{\prog,\predset}(I) = \mu \predtrans. \bigcup_{\trn \in \edges} \operatorname{post}_{\trn,\predset} (\predtrans) \cup I$.
%  The \emph{initial abstraction} is the set of predicate transitions $I_{\prog,\predset,\pi} = \{(\pi,\alpha_\predset(\trn),\loc) \mid (\pi,\trn,\loc) \in \prog \}$.
%  For a set of predicate transitions $\predtrans$ we denote by $\predtrans |_\pi = \{ p \mid (\pi,p,\pi) \in \predtrans \}$ its \emph{restriction to $\pi$}.
%  The \emph{transition predicate abstraction} $TPA_{\predset,\prog,\pi} = \operatorname{lfp}_{\prog,\predset}(I_{\prog,\predset,\pi}) |_\pi$ is the least fixed point of the post operator w.r.t. the initial abstraction restricted to $\pi$.
%\end{definition}

%In the next lemma we state that transition predicate abstraction computes transition invariants.
%
%\begin{lemma}[\cite{conf/popl/PodelskiR05}]
%  $\transinv_{\predset,\prog,\loc}$ is a forward invariant for $\prog|_\loc$.
%\end{lemma}

%We now compare TPA to our SCA approach by looking at the program from Example~\ref{ex:abstraction} for which we want to compute a transition invariant for $\loc_1$.
%
%TPA starts by abstracting the transition $(\loc_1, \trn_1,\loc_2)$ to $(\loc_1, \alpha_\predset(\trn_1),\loc_2)$ and iterates through the inner loop until the set of predicate transitions stabilizes:
%$\predtrans_1 =  \operatorname{post}_{\loc_2 \xrightarrow{\trn} \loc_2,\predset}(I_{\prog,\predset,\pi})$,
%$\predtrans_2 =  \operatorname{post}_{\loc_2 \xrightarrow{\trn} \loc_2,\predset}(\predtrans_1)$,
%...,
%$\predtrans_{k+1} =  \operatorname{post}_{\loc_2 \xrightarrow{\trn} \loc_2,\predset}(\predtrans_k)$ and $\predtrans_k = \predtrans_{k+1}$.
%Then TPA computes $\predtrans_{k+2} =  \operatorname{post}_{\loc_2 \xrightarrow{\trn_2} \loc_1,\predset}(\predtrans_{k+1})$ and reaches the header of the outer loop $\loc_1$.
%TPA iterates through the outer loop until the set of predicate transitions stabilizes, in particular it can not conclude that the fixed point is reached after the first iteration:
%$\predtrans_{k+3} =  \operatorname{post}_{\loc_1 \xrightarrow{\trn_1} \loc_2,\predset}(\predtrans_{k+2})$, ...,
%TPA analyses again the inner loop, goes back to $\loc_1$, and so on, until a fixed point is reached.

%At every step in the fixed point construction of $\edges_{TPA,\predset,\prog}$ precision can be lost, as the inequality
%\begin{displaymath}
%  \gamma(\preds) \circ \trn \subseteq \gamma(\alpha_\predset(\gamma(\preds) \circ \trn))
%\end{displaymath}
%is strict in general! In particular TPA can lose information during the computation of the transitive hull of a loop and on paths when intermediate predicates are missing.
%The crucial difference to our SCA approach is that we lose precision only when abstracting summarized inner loops.
%Before we abstract loops we refine their control flow such that the subsequent abstraction is precise enough.
%The computation of transitive hulls is done precisely within SCA.
%For paths we do not lose precision as our pathwise analysis implicitly includes all intermediate predicates in the SMT solver queries by which we construct the abstraction.
%
%
%The size-change abstraction enjoys a completeness property w.r.t. termination which we state after the following definition.
%
%
%\begin{lemma}
%  Let $\scrset \subseteq \scrs$ be an SCR set.
%  $\scrset$ is terminating, iff $\scrset^+$ is terminating.
%\end{lemma}
%
%TPA is not associative. Because of that we abstract pathwise.


%\cite{conf/lics/PodelskiR04, conf/cav/KroeningSTW10} are model checking based approaches.
%The cited works do not explain how they extract the transition predicates.
%Furthermore transition predicate abstraction looses precision at every step of the fixed point computation until a fixed point is reached.
%Because of both reasons it is unclear how to reimplement their approaches and to get an intuition about what they can prove in practice.
%In comparison to this we are very explicit on what kind of predicates we use.
%The intuition underlying our methodology is easy to grasp:
%we rely on the assumption that there are linear increases or decreases of some norms on the program state.

%1. During the analysis of the inner loop we lose precision only at the one point of time when we abstract its transition relations to SCRs.
%Before we abstract we refine the control flow of the inner loop such that the transformed loop has a clear behavior on increasing or decreasing norms.
%After the refinement we do not want to keep any other information than norm increases or decreases and apply SCA in order to abstract the non-relevant information.
%Then we apply the transitive hull computation on SCRs in order to get the dynamics of the norms when different paths of the inner loop interact.
%Computing the hull on SCRs does not lose precision.
%In this way we extract only the relevant information from the inner loop.
%
%2. After the summarization of the inner loop by its transitive hull, control flow refinment is called on the outer loop with header $\loc_1$.
%First all paths from header to header are contracted, then the loop is unrolled and finally contextualized.
%All these steps happen without loss of precision.
%After that the outer loop is abstracted to an SCS $\scs$  and directly anaylzed for ranking functions / bounds.
%The difference between SCA and TPA is that TPA does not use control flow refinement but goes on until if reaches a fixed point, which is a transition invariant for $\loc_1$.
%
%From a methodological point of view we can explain this is follows:
%$\scs$ is a generator of the transitive hull $\scs^+$, which can can be computed in finitely many steps from $\scs$ without any loss of precision.
%Thus we also use transition invariants but without explicitly computing them!
%Thus analyzing $\scs$ directly for ranking functions / bounds is as precise as analyzing the transition invariant $\scs^+$ but less costly.



\subsection{Termination Analysis by {\sc Loopfrog}}
\label{subsec:loopfrog}

\cite{conf/cav/KroeningSTW10,conf/tacas/TsitovichSWK11} observe that TPA-based approaches such as {\sc Terminator}~\cite{conf/pldi/CookPR06} spend almost all time in analyzing the transitive hulls of programs, i.e., the expensive step is proving $\prog|_\loc^+ \subseteq \bigcup \transinv$ for transition sets $\transinv$.
Therefore~\cite{conf/cav/KroeningSTW10,conf/tacas/TsitovichSWK11} take a different approach and give algorithms that search for a transitive transition system $\transinv$ for $\prog|_\loc$.
A transition set $\transinv$ is \emph{transitive}, if $\bigcup \transinv^2 \subseteq \bigcup \transinv$.
A transitive transition system $\transinv$ for $\prog|_\loc$ already implies $\prog|_\loc^+ \subseteq \bigcup \transinv^+ \subseteq \bigcup \transinv$ by the transitivity of $\transinv$.
This has the advantage that the expensive direct proof of $\prog|_\loc^+ \subseteq \bigcup \transinv$ is avoided.

The first version of {\sc Loopfrog}~\cite{conf/cav/KroeningSTW10} implements an algorithm that constructs such transitive transition systems iteratively.
In every step {\sc Loopfrog} adds transition relations to a candidate transition set $\transinv$.
We argue that the effectiveness of such an iterative algorithm is limited, and that what the authors of \cite{conf/cav/KroeningSTW10} really want is SCA!

%The authors of~\cite{conf/cav/KroeningSTW10} argue on their example program~\ref{ex:kroening} in their section 4.3 that the transition set $\transinv_1 = \{\scr_1,\scr_2\}$ with $\scr_1 = x \mod 2 \neq 0 \wedge x > x^\prime \wedge x \mod 2 = 0$ and $\scr_2 = x < 255 \wedge x < x^\prime$ is a transitive d.wf. transition invariant because $\prog^2 \setminus \transinv_1 \subseteq \transinv_1$ can be proved.
%% and thus termination is concluded according to the above cited prove rule.
%However, this argumentation is flawed because proving $\prog^2 \setminus \transinv_1 \subseteq \transinv_1$ does not suffice to show that $\transinv_1$ is transitive.
%In fact $\transinv_1$ contains the pairs $(1,0)$ and $(0,1)$, which allows an infinite alternation between $1$ and $0$.
%Thus the d.wf. transition set $\transinv_1$ can not be transitive, because transitivity and d.wf. imply well-foundedness.

Note that a transitive transition system $\transinv$ for $\prog|_\loc$ that is precise enough to prove the termination of $\prog$ is an overapproximation of $\prog$ that still terminates.
%Therefore once the candidate transition set $\transinv$ does not terminate, it cannot be repaired by adding transition relations.
%Next we argue why $\transinv$ cannot be found iteratively.
Let us consider an example transition set $\transinv = \{\trn_1,\trn_2\}$ with $\trn_1 = x > 0 \wedge x > x^\prime$ and $\trn_2 = y > 0 \wedge y > y^\prime$.
$\transinv$ does not terminate because $\trn_1$ can increase the value of $y$ arbitrarily and $\trn_2$ can increase the value of $x$ arbitrarily.
Let us assume that the analyzed program $\prog$ nevertheless terminates because the variable $x$ can only be decreased when $y$ stays constant.
Let us further assume that {\sc Loopfrog} has added $\trn_1$  to $\transinv$ in the first step and $\trn_2$ in the second step of its iteration.
{\sc Loopfrog} could have added the information about $x$ in the first step by setting $\trn_1 = x > 0 \wedge x > x^\prime \wedge y = y^\prime$, but not in the second step.
%Observe that the transition relations of $\transinv$ terminate, when considered in isolation.
Note that once the candidate transition set $\transinv$ does not terminate, it cannot be repaired by adding transition relations.
Note further that in later steps the loss of information of earlier steps cannot be repaired as we have seen on the above example.
Thus, we conclude that a candidate transition set $\transinv$ has to be constructed in one single step.
This is exactly what we do in our analysis.
We first compute transition system for programs, and then size-change abstract the transition relations for our bound analysis.
Alternatively, these abstracted transition relations could be analyzed for termination by a transitive hull computation using the termination criterion of SCA~\cite{mcs-integers}.
This transitive hull then provides exactly the transitive transition system $\transinv$ for $\prog|_\loc$.
From this we conclude that what the authors of \cite{conf/cav/KroeningSTW10} really want is SCA!

%The transitivity and d.wf. of $Q_{k_2}$ would imply the well-foundedness of $Q_{k_2}$, what is a contradiction to $Q_{k_1} \subseteq Q_{k_2}$.
%2. The cited iterative proof rule suggests that progress is made and that $Q_k$ is closer to a transitive d.wf. transition invariant for higher values of $k$.
%However, this is not the case under reasonable assumptions (details omitted
%due to space restrictions.)
%that the abstraction function $\alpha$ used to construct the constituent relation of the d.wf. transition invariant has the property $\alpha(\trn_1 \circ \trn_2) \subseteq \alpha(\trn_1) \circ \alpha(\trn_2)$ for all relations $\trn_1,\trn_2$.
%Assume that as in the above case the loop $\prog = \{\trn_1,\ldots,\trn_n\}$ is abstracted to a d.wf. transition set $\transinv_1 = \{\scr_1,\ldots,\scr_n\}$ with $\scr_i = \alpha(\trn_i)$.
%The $k$ times unrolled $\prog^k = \{\trn_{j_1} \circ \cdots \circ \trn_{j_k} \mid j_i \in \{1,\ldots,n\} \}$ contains all $k$-fold concatenations of the transition relations.
%We get that the abstraction of every such a $k$-fold concatenation $T = \alpha(\trn_{j_1} \circ \cdots \circ \trn_{j_k} \subseteq \alpha(\trn_{j_1}) \circ \cdots \alpha(\trn_{j_k}) = \scr_{j_1} \circ \cdots \circ \scr_{j_k} \subseteq \transinv_1^k$ is already contained in $Q_1^k$.
%Adding all such $T$'s to $\transinv_k$ does not get closer to a transitive d.wf. transition invariant because we have $\transinv_k \subseteq Q_1^k$ for every $k$.
%The distinction with our unrolling technique of Section~\ref{subsec:unrolling} is that when unrolling $\{\trn_1,\trn_2\}$ to $\{\trn_1 | \trn_2\trn_1 | \trn_2\trn_2\}$ we `delete' $\trn_2$ but \cite{conf/cav/KroeningSTW10} `keeps' $\trn_2$ and therefore does not win precision.
%3. From 1. and 2. we see that a transitive d.wf. transition invariant has to be found by a single abstraction.
%As described above $\transinv_1  = \{\scr_1,\scr_2\}$ is not transitive.
%What has gone wrong?
%\cite{conf/cav/KroeningSTW10} follows~\cite{conf/pldi/CookPR06} and constructs a ranking function for single transitions.
%For example, if $rank$ is a ranking function for a transition $\rho$, i.e., $\rho \subseteq rank > 0 \wedge rank > rank^\prime$, then $\rho$ is abstracted to the well-founded transition $\scr = rank > 0 \wedge rank > rank^\prime$.
%Simply taking the union of such abstractions as a transition invariant does not work as the abstractions also need to incorporate the information how the values of the ranking functions of the respective other transitions are altered.
%%
%%can be seen on $\transinv_1$.
%%This is because the abstraction also needs to contain the information how the values of the ranking functions behave on different transitions.
%%In Example~\ref{ex:kroening} there is no cyclic dependency because $\trn_1$ can be executed only once, which is captured by our technique of contextualization.
%To be specific we look at the transition invariant $\transinv = \{\scr_1,\scr_2\}$ with $\scr_1 = x > 0 \wedge x > x^\prime$ and $\scr_2 = y > 0 \wedge y > y^\prime$.
%Note that $\transinv$ is not well-founded because $\scr_1$ can increase $y$ arbitrarily and $\scr_2$ can increase $x$ arbitrarily.
%More information has to be included in the abstraction, for example if $\trn_1$ can not increase $y$ we can choose $\scr_1 = x > 0 \wedge x > x^\prime \wedge y \ge y^\prime$, what makes $\transinv$ transitive.
%The description of how the values of local ranking functions change on the different transitions can be done very naturally in the SCA framework!

%Our experiments confirm the observation of~\cite{conf/cav/KroeningSTW10} that using transitive transition invariants achieve a speedup over the TPA fixed point computation approach underlying~\cite{conf/pldi/CookPR06}.

%To sum up the SCA framework correctly implements the idea of~\cite{conf/cav/KroeningSTW10} on using transitive transition invariants for achieving a speedup over the TPA fixed point computation approach underlying~\cite{conf/pldi/CookPR06}.
%The speedup is also confirmed by our experiments, which show that we get a scalable solution that can analyze huge codesbases in practice.

%\subsection{TPA Example}
%
%We explain on the following example how predicate abstraction works.
%We will use this example later to explain the difference to SCA.
%
%\begin{verbatim}
%while(x != 0)
%if (x > 0)
%    x--;
%else
%    x++;
%\end{verbatim}
%
%We have two transitions:
%\begin{itemize}
%\item $\trn_1 \equiv x > 0 \wedge x^\prime = x-1$
%\item $\trn_2 \equiv x < 0 \wedge x^\prime = x+1$
%\end{itemize}
%
%Consider transition predicate abstraction with the sets $P_1=\{x>0,x<0,x^\prime > x,x^\prime < x$ and $P_2=\{x>0,x<0,x^\prime = x - 1,x^\prime = x + 1,x^\prime > x,x^\prime < x$.
%
%Assume the four transition invariants $\scr_1 = x > 0 \wedge x^\prime > x$, $\scr_2 = x < 0 \wedge x^\prime < x$, $\scr_3 = x > 0 \wedge x^\prime = x-1$, and $\scr_4 = x > 0 \wedge x^\prime = x+1$.
%
%$P_1$ gives us the following proof:
%\begin{displaymath}
%start \xrightarrow{\trn_1} \scr_1, \scr_1 \xrightarrow{\trn_1} \scr_1, \scr_1 \xrightarrow{\trn_2} \scr_1, start \xrightarrow{\trn_2} \scr_2, \scr_2 \xrightarrow{\trn_2} \scr_2, \scr_2 \xrightarrow{\trn_2} \scr_2
%\end{displaymath}
%
%$P_2$ gives us the following proof:
%\begin{displaymath}
%start \xrightarrow{\trn_1} \scr_3, \scr_3 \xrightarrow{\trn_1} \scr_1, \scr_1 \xrightarrow{\trn_1} \scr_1, \scr_1 \xrightarrow{\trn_2} \scr_1, start \xrightarrow{\trn_2} \scr_4, \scr_4 \xrightarrow{\trn_2} \scr_2, \scr_2 \xrightarrow{\trn_2} \scr_2, \scr_2 \xrightarrow{\trn_2} \scr_2
%\end{displaymath}
%Note that there is no transition from $\scr_3$ by $\trn_2$ because the conjunction $\scr_3 \wedge \trn_2^\prime$ is unsatisfiable. The same holds for $\scr_4$ and $\trn_1$.
%
%TODO: Explain the connection of these two cases with the missing example from~\cite{conf/sas/HeizmannJP10}.
%
%Consider the following program, which cannot be proved by $P_1$ or $P_2$, but which has the same transition invariant $\scr_1 \cup \scr_2$:
%\begin{itemize}
%\item $\trn_1 \equiv x > 0 \wedge x^\prime > x \wedge y^\prime = x$
%\item $\trn_2 \equiv x < 0 \wedge x^\prime < x \wedge x^\prime < y \wedge y^\prime = y$
%\end{itemize}

%\vspace*{-2mm}
The second version of {\sc Loopfrog}~\cite{conf/tacas/TsitovichSWK11} uses relational loop summarization (see also the next subsection).
For this summarization~\cite{conf/tacas/TsitovichSWK11} uses template invariants.
Only one of these templates contains disjunction (two disjuncts).
\cite{conf/tacas/TsitovichSWK11} states that these templates are inspired by the more general size-change abstract domain.
We show in this paper how to employ the full SCA domain by using pathwise analysis for exploiting the looping structure of imperative programs.
This allows us to use the full disjunctive power of SCA.
\cite{conf/tacas/TsitovichSWK11} is only concerned with termination analysis, whereas we show how to use SCA for the more difficult problem of bound analysis.
%We give two program transformations that make our analysis more precise, whereas \cite{conf/tacas/TsitovichSWK11} does not give such transformations.

\subsection{Loop Summarization}

Loop summarization as in Algorithm~\ref{alg:transitionSystem} is being recognized as important tool in program analysis, for example~\cite{conf/atva/KroeningSTTW08} summarizes loops by overapproximations of the reachable states for automatic proofs of safety properties.
Relational summarizations of loops have for the first time been used in the bound analysis of~\cite{conf/pldi/GulwaniZ10}.
The termination analysis~\cite{conf/tacas/TsitovichSWK11}, which is an extension of~\cite{conf/atva/KroeningSTTW08}, also uses relational summaries of loops.

Loop summarization is closely related to procedure summarization, e.g.~\cite{conf/esop/GulwaniT07}.

\subsection{Disjunctive Abstract Domains}
\label{subsec:disjunction-abstract-domains}

The papers~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07} on bound and termination analysis use abstract interpretation for computing disjunctive transition invariants.
Both papers suggest lifting a conjunctive abstract domain $D$ to the powerset domain $2^D$,
and refer to the standard octagon / polyhedra domains as instantiations of $D$ in their implementation sections.

However, lifting the octagon / polyhedra domain to the powerset domain is difficult because it requires an adequate lifting of the join operator:
Set union is the precise join operator of both powerset lattices, but every set union may increase the number of the base elements of the powerset elements.
Note that both powerset lattices have infinite width.
Thus using set union as join operator does not guarantee the termination of the analysis.
A standard way of ensuring the finiteness of the analysis is by limiting the number of base elements of a powerset element, such that every time the number of base elements of a powerset element is over the limit some base elements are merged.

\cite{conf/pldi/GulwaniZ10} states an algorithm for lifting the join operator to the powerset domain based on an assumption resembling convex theories that uses the same syntactic merging function in every step of the fixed point computation.
However, \cite{conf/pldi/GulwaniZ10} proposes to choose the merging function heuristically or to try all merging functions for a small number of disjuncts and take the best result.
%For a small number of disjuncts it is possible to enumerate the results of all merging functions and for a larger number the merging function has to be constructed by a heuristic.
\cite{conf/popl/BerdineCCDO07} remains vague: ``For our present empirical evaluation we use an extraction method after the fixed-point analysis has been performed in order to find disjunctive invariance/variance assertions.''.

%SCA is a finite subset of the powerset domain of the octagon / polyhedra domain (the number of SCRs is finite).
In contrast, SCA is a finite powerset domain that naturally handles disjunction:
SCA has finite width, therefore we never have to merge abstract elements and can handle disjunction precisely.
This releases us from relying on complicated merging algorithms as~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07}.
SCA has finite height, therefore we do not need widening to compute fixed points (e.g. transitive hulls).
This releases us from lifting the widening operator of conjunctive domains (e.g. octagon, polyhedra) to powerset domains.
%Because of these features we are convinced that SCA is the right abstract domain for handling disjunction in termination / bound analysis.

\subsection{Bound Analysis by the {\tt SPEED} project}
\label{subsec:speed}

In earlier work~\cite{conf/pldi/GulwaniZ10} we have stated proof rules for computing global bounds from local bounds of transitions. % that were motivated by the examples they found throughout their experiments.
Ad hoc proof rules as in~\cite{conf/pldi/GulwaniZ10} often give rise to efficient analyses, but do not establish a general theory. % in which the problem can be placed.
This is unsatisfying because such a theory is crucial for investigating the completeness of the analysis and the applicability to related problems or other programming paradigms.
In this paper we have identified SCA as a suitable abstraction for bound analysis.
SCA provides the theory that we have been looking for, because all the proof rules of~\cite{conf/pldi/GulwaniZ10} are instantiations of our more general bound algorithm.

In~\cite{conf/pldi/GulwaniZ10} we stated a so-called \emph{enabledness} check that detects non-interference between transitions, which can be used in the composition of the global bound.
Unfortunately, this check is flawed when more than two transitions are considered.
Our program transformation contextualization can soundly detect non-interference when an arbitrary number of transitions is considered.

%\item {\sc SPEED} restricts every transition to having only one ranking function.
%By following SCA we are able to take multiple ranking functions per transition into account .
%\item By borrowing the calling-context graph technique from the size-change literature we are able to handle loops that we could not be handled before.
%\item We treat multiple ranking functions at the same times.
%    This has the advantage that we compute a bound where we could not compute a bound before, or where we compute a better bound.
%    We can compute multiple bounds, e.g. the minimum of a linear and a multiplicative bound.
%    When expressing the bounds in terms of the input variables some of these bounds can not be expressed in this way.
%    Therefore it is beneficial to have multiple bounds.
%    Moreover the quality of the bounds also becomes clear only after expressing them in terms of the input.
%    All this is enabled by an efficient ranking function computation.

\cite{conf/pldi/GulwaniJK09} proposes to use program transformation before performing bound analysis.
The program transformation stated in~\cite{conf/pldi/GulwaniJK09} is parameterized by an abstract domain, which is used simultaneously with the actual transformation algorithm to detect the infeasibility of certain paths.
However, \cite{conf/pldi/GulwaniJK09} is vague about what abstract domains should be used, and the actual transformation algorithm is quite involved.
In contrast, we propose two simple program transformations that are easy to implement.
Our program transformations only rely on SMT solver calls and do not require additional abstract domains.

%\vspace*{-2mm}

\subsection{Size-change Abstraction}
\label{subsec:sca}

%\TODO{Im neuen Paper ?} and preconditions for non-termination can be computed
%    Furthermore in current work we show that the abstraction also allows to extract bounds and that these bounds are polynomial in the initial values of the variables.
%\end{itemize}
%
%
%Most previous research on SCA, e.g.~\cite{conf/popl/LeeJB01,mcs-integers}, has focused on the abstract model and its properties and has no yet answered the question how to abstract programs.
%A notable exception is the work by Manolios et al.~\cite{conf/cav/ManoliosV06}, which integrates SCA and the theorem proving capabilities of ACL2 to prove termination of over 98\% of the 10,000+ functions in the ACL2 regression suite without user guidance~\cite{conf/cav/ManoliosV06}.

Despite its success in functional/declarative languages, e.g.~\cite{conf/cav/ManoliosV06}, \cite{conf/cade/Krauss07}, SCA~\cite{conf/popl/LeeJB01,mcs-integers} has not yet been applied to imperative programs.
We describe the two main obstacles in the application of SCA to imperative programs and how we solve them:
%
(1) In functional / declarative languages, algorithms typically operate on algebraic data structures where constructs and destructs happen in single steps.
Due to this succinctness, SCA achieves sufficient precision on small program blocks.
In imperative programs loops can have many intermediate stages and oftentimes only the program state at the loop header can be considered as ``clean''.
Therefore the abstraction of small program blocks to size-change relations loses too much precision.
(This issue is well-known in the field of invariant computation.)
We solve this issue by our pathwise analysis, which has the effect that large pieces of code that lie between the ``clean'' program locations are abstracted jointly.
%
(2) The intended use of the SCA variables is as {\em local progress measures of the program.}
In functional/declarative languages there is a natural set of such local progress measures such as the size of a data type, the height of a tree, the length of a list, or any arithmetic expression built up from those.
In imperative programs, it is less clear what the shape of this local progress measures is and how they can be automatically extracted from programs.
%The naive reuse of integer program variables as SCA variables might fall short of capturing the progress properties of the program.
We give a solution to this problem by extracting norms from the conditions of complete loop paths (as described in our heuristics).

%We will also sketch a way how to handle complex data structures.

%Full elaboration of~\cite{mcs-integers} is a program transformation that separates control from transition invariants.

\subsection{Other Approaches}

A series of works describes a type-based potential-method of amortized analysis for the estimation of resource usage in first-order functional programs, which reduces the problem to linear constraint solving.
Recent enhancement includes the extension to multivariate polynomial bounds~\cite{conf/popl/HoffmannAH11} and higher-order programs~\cite{conf/popl/JostHLH10}.

The embedded and real-time systems community has taken considerable effort on
worst case execution time (WCET) estimation~\cite{journals/tecs/WilhelmEEHTWBFHMMPPSS08}.
WCET presents an orthogonal line of research, which for establishing loop bounds either requires user annotations or employs simple techniques based on pattern matching and numerical analysis.
We report on a WCET benchmark in our experiments.

%It would be interesting to implement the SCA approach in a lazy abstraction framework such as {\tt Terminator} (compare recent publication by Jones et al.~\cite{conf/sas/HeizmannJP10}).

%Manolios and Vroon~\cite{conf/cav/ManoliosV06} used concatenation only on transitions that have just one successor transition.



%Our experiments show that we can get a scalable solution:
%\begin{itemize}
%\item On C-code, whereas the experiments of the experiments of {\sc SPEED} were on .net code.
%\item As the proposed approach is strictly more general - as we will demonstrate later - we can show that the methodology works on C-code and .net code found in practice.
%\item Our experiments were executed on benchmarks from the WCET community as well as on cBench.
%\end{itemize}

%\vspace*{-8mm} 

==> include/conclusion.tex <==
\svnid{$Id$}
\section{Conclusion}

\todo{NEEDS UPDATE TO MATCH THE INTRO}

We have demonstrated that SCA is a highly effective framework for termination
and bound analysis of imperative programs. SCA offers a clear separation of concerns between control invariants and transition invariants. We showed how to exploit this separation of concerns for computing more precise bounds than previous techniques with a simpler methodology. Furthermore we presented several techniques such as path-wise abstraction and contextualization that make the abstraction process sufficiently precise.

\todo{REST MOVED FROM INTRO}

We believe that identifying SCA as the right abstract domain for bound analysis of imperative programs is a main contribution of this paper.
We view our solution as one choice in the solution space offered by this powerful abstraction framework.
Further investigations on SCA are worthwhile, for example, our bound algorithm is a simple greedy algorithm, which handles many programs occurring in practice, but which does not exploit the full power of SCA.




Most existing research on the termination/bound problem has been divided into separate lines for the imperative and functional/declarative world.
Our work for the first time bridges this gap by using SCA in an imperative setting. We hope that our paper will foster the transfer of ideas and techniques between these areas. We give the first example of such a cross-fertilization by using the program transformation contextualization
which was originally developed for functional programs~\cite{conf/cav/ManoliosV06}.

However, we want to stress that there is ample space for in-depth investigations on the sweet spot between precision and speed. Our solution is but one choice in the solution space offered by this powerful abstraction framework.


==> include/excluded.tex <==
\begin{verbatim}
// cBench/consumer_tiff2bw/tif_luv.c
// Decode a string of 16-bit gray pixels.
static int
LogL16Decode(TIFF* tif, tidata_t op, tsize_t occ,
tsample_t s)
{
  LogLuvState* sp = DecoderState(tif);
  int shft, i, npixels;
  u_char* bp;
  int16* tp;
  int16 b;
  int cc, rc;

  assert(s == 0);
  assert(sp != NULL);

  npixels = occ / sp->pixel_size;

  if (sp->user_datafmt == SGILOGDATAFMT_16BIT)
    tp = (int16*) op;
  else {
    assert(sp->tbuflen >= npixels);
    tp = (int16*) sp->tbuf;
  }
  _TIFFmemset((tdata_t) tp, 0, npixels*sizeof (tp[0]));

  bp = (u_char*) tif->tif_rawcp;
  cc = tif->tif_rawcc;
              /* get each byte string */
  for (shft = 2*8; (shft -= 8) >= 0; ) {
    for (i = 0; i < npixels && cc > 0; )
      if (*bp >= 128) {		/* run */
        rc = *bp++ + (2-128);
        b = (int16)*bp++ << shft;
        cc -= 2;
        while (rc--)
          tp[i++] |= b;
      } else {			/* non-run */
        rc = *bp++;		/* nul is noop */
        while (--cc && rc--)
          tp[i++] |= (int16)*bp++ << shft;
      }
    if (i != npixels) {
      TIFFError(tif->tif_name, "LogL16Decode:
      Not enough data at row %d (short %d pixels)", tif->tif_row, npixels - i);
      tif->tif_rawcp = (tidata_t) bp;
      tif->tif_rawcc = cc;
      return (0);
    }
  }
  (*sp->tfunc)(sp, op, npixels);
  tif->tif_rawcp = (tidata_t) bp;
  tif->tif_rawcc = cc;
  return (1);
}
\end{verbatim}


We are interested in how often the inner for loop can be executed.
We abbreviate the integer variables {\tt shift} and {\tt npixels} by $s$ and $n$.

\begin{itemize}
\item $\rho_1 \equiv i < n \wedge cc > 0 \wedge cc^\prime = cc - 2 \wedge i^\prime > i$
\item $\rho_2 \equiv i < n \wedge cc > 0 \wedge cc^\prime > cc  \wedge i^\prime > i$
\item $\rho_3 \equiv i < n \wedge cc > 0 \wedge cc^\prime = cc - 2 \wedge i^\prime = 0$
\end{itemize} 

An example from our experiments shows how unrolling can be used to increase the precision of our analysis even in the presence of contextualize.

\begin{verbatim}
// cBench\consumer_jpeg_c\src
// function: h2v2_fancy_upsample

while (outrow < cinfo->max_v_samp_factor)
    for (v = 0; v < 2; v++)
        outrow++;
\end{verbatim}


Analyzing the for loop in the above function gives us the following two transitions $\trn_1, \trn_2$,
where we abbreviate {\tt outrow} by $o$ and {\tt cinfo->max\_v\_samp\_factor} by $end$:
\begin{itemize}
\item $\trn_1 \equiv v < 2 \wedge v^\prime = v+1 \wedge o^\prime = o+1$
\item $\trn_2 \equiv v \ge 2 \wedge v^\prime = 0 \wedge o < end$
\end{itemize}

Abstracting the program directly to a size-change program would result in the transitions $T_1$ and $T_2$ which are not sufficient to prove program termination:
\begin{itemize}
\item $T_1 \equiv v < 2 \wedge v^\prime > v \wedge o^\prime > o$
\item $T_2 \equiv v \ge 2 \wedge v^\prime = 0 \wedge o < end$
\end{itemize}

After contextualization we get the following control flow graph involving the two locations $f_1$ and $f_2$:
\begin{displaymath}
f_1 \xrightarrow{T_1} f_1, f_1 \xrightarrow{T_2} f_2, f_2 \xrightarrow{T_1} f_1
\end{displaymath}

Note that we still can not prove termination by the size-change abstraction.
This is because the only ranking function for $T_1$ is $1-v$, and the only ranking function for $T_2$ is $v-2$ (integer or bool).
Each transition increases the value of the other transition, therefore the termination check fails.
The problem is transition $T_1$ increases $o$ and $T_2$ checks that $o$ does not exceed its upper bound $end$.
However this information is not taken into account as every transition on its own has to decrease.
With unrolling we are able to handle the example.

However by unrolling $\trn_1 | \trn_2$ to $\trn_1 | \trn_2\trn_1 | \trn_2\trn_2$ we obtain the program:
\begin{itemize}
\item $\trn_1 \equiv v < 2 \wedge v^\prime = v+1 \wedge o^\prime = o+1$
\item $\trn_2\trn_1 \equiv v \ge 2 \wedge o < end \wedge v^\prime = 1 \wedge o^\prime = o+1$
\end{itemize}
Note that $\trn_2\trn_2$ is omitted because it is not satisfiable.

Abstracting the unrolled program results in a size-change abstraction which can prove termination:
\begin{itemize}
\item $T_1 \equiv v < 2 \wedge v^\prime > v \wedge o^\prime > o$
\item $T_{21} \equiv v \ge 2 \wedge o < end \wedge v^\prime = 1 \wedge o^\prime > o$
\end{itemize}


==> include/experiments.tex <==
\svnid{$Id$}
\vspace{-0.4cm}
\section{Experiments}
\label{sec:experiments}
\vspace{-0.2cm}

Our tool {\sc Loopus} applies the methods of this paper to obtain upper bounds on loop iterations. The tool employs the LLVM compiler framework and performs its analysis on the LLVM intermediate representation~\cite{llvm}.
We are using ideal integers in our analysis instead of exact machine representation (bitvectors).
Our analysis operates on the SSA variables generated by the mem2reg pass and handles memory references using optimistic assumptions.
For logical reasoning we use the {\em yices} SMT solver \cite{yices}.
Our experiments were performed on an Intel Xeon CPU (4 cores with 2.33 GHz) with 16 GB Ram.
{\sc Loopus} computed a bound for 93\% of the 262 loops of the M\"alardalen WCET \cite{wcetbench} benchmark (72\% for loops with more than one path) in less than 35 seconds total time.
{\sc Loopus}  computed  a bound for 75\% (65\% for loops with more than one path) of the 4090 loops of the compiler optimization benchmark cBench \cite{cbench} within a 1000 seconds timeout for each loop (3923 loops in less than 4 seconds).
1102 of the 4090 loops required the summarization of inner loops.
{\sc Loopus} computed a bound for 56\% of these loops.
We give more details about our experiments and the cases in which we failed in the extended version of this paper. %Section~\ref{sec:experiments-appendix} of the appendix.

\vspace{0.2cm}

\textbf{Acknowledgement.} We would like to thank the anonymous reviewers for their insightful comments. 

==> include/introduction-new.tex <==
\svnid{$Id$}

\section{Introduction}

%\vspace{-0.2cm}

%Structure:
%- what is the problem and why is it important
%- what are the difficulties in solving it
%- what is our solution
%- why does it solve the difficulties
%- how does it compare to the approaches from the literature


% introduction and importance of the bound problem
Computing symbolic bounds for the resource consumption of imperative programs is an active area of research~\cite{conf/pldi/GulwaniZ10,conf/popl/GulwaniMC09,conf/pldi/GulwaniJK09,conf/cav/Gulwani09,conf/cav/GulavaniG08,conf/sigsoft/GoldsmithAW07}. Most questions about resource bounds can be reduced to counting the number of visits to a certain program location~\cite{conf/pldi/GulwaniZ10}.
Our research is motivated by the following technical challenges:

%\smallskip

\noindent{\bf (A)} Bounds are often {\em complex non-linear arithmetic expressions} built from $+,*,\max$ etc.
Therefore, abstract domains based on linear invariants (e.g.~intervals, octagons, polyhedra) are not directly applicable for bound computation.

%\smallskip

\noindent{\bf (B)} The proof of a given bound often requires {\em disjunctive invariants} that can express loop exit conditions, phases, and flags which affect program behavior.
Although recent research made progress on computing disjunctive invariants~\cite{conf/pldi/GulwaniZ10,conf/pldi/GulwaniJK09,conf/lics/PodelskiR04,conf/pldi/CookPR06,conf/popl/BerdineCCDO07,conf/asian/PopeeaC06,Reps06}, this is still a research challenge.
(Note that the domains mentioned in (A) are conjunctive.)


%\smallskip

\noindent{\bf (C)} It is {\em difficult to predict a bound in terms of a template} with parameters because the search space for suitable bounds is huge.
Moreover the search space cannot be reduced by compositional reasoning because bounds are global program properties.

%\smallskip

\noindent{\bf (D)} It is not clear how to {\em exploit the loop structure} to achieve compositionality in the analysis for bound computation.
This is in contrast to automatic termination analysis where the cutpoint technique~\cite{conf/pldi/CookPR06,conf/popl/BerdineCCDO07} is used standardly.

In this paper we demonstrate that the size-change abstraction (SCA)~by Lee et al.~\cite{conf/popl/LeeJB01,mcs-integers} is the right abstract domain to address these challenges. SCA is a predicate abstraction domain that consists of (in)equality constraints between integer-valued variables and boolean combinations thereof in disjunctive normal form (DNF).
%The inequality constraints consist of \emph{control predicates} which describe control invariants and \emph{transition predicates} which describe transitions of the program state.
%the monotonic change (increase, constant, or decrease) of the variables incurred by a computation.

SCA is well-known to be an attractive abstract domain: First, SCA is rich enough to capture the progress of many real-life programs. It has been successfully employed for automatic termination proofs of recursive functions in functional and declarative languages, and is implemented in widely used systems such as ACL2, Isabelle etc.~\cite{conf/cav/ManoliosV06,conf/cade/Krauss07}.
Second, SCA is simple enough to achieve a good trade-off between expressiveness and complexity. For example, SCA termination is decidable and ranking functions can be extracted on terminating instances in PSPACE~\cite{mcs-integers}. The simplicity of SCA sets it apart from other disjunctive abstract domains used for termination/bounds such as transition predicate abstraction~\cite{conf/popl/PodelskiR05} and powerset abstract domains~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07}.

Our method starts from the observation that progress in most software depends on the {\em linear change} of integer-valued functions on the program state (e.g., counter variables, size of lists, height of trees, etc.), which we call \emph{norms}. The vast majority of non-linear bounds in real-life programs stems from two sources -- nested loops and loop phases -- and not from inherent non-linear behavior as in numeric algorithms. For most bounds, we have therefore the potential to exploit the nesting structure of the loops, and compose global bounds from bounds on norms. Upper bounds for norms typically consist of simple facts such as size comparisons between variables and can be computed by classical conjunctive domains. SCA is the key to convert this observation into an efficient analysis:

\noindent {\bf (1)} Due to its built-in disjunctiveness and the transitivity of the order relations, SCA is closed under taking transitive hulls, and transitive hulls can be efficiently computed. We will use this for summarizing inner loops.

\noindent {\bf (2)} We use SCA to compose global bounds from bounds on the norms.
To extract norms from the program, we only need to consider small program parts.
After the (local) extraction we have to consider only the size-change-abstracted program for bound computation.
%A similar separation of concerns has been used for termination analysis in the {\sc Terminator} tool~\cite{conf/pldi/CookPR06} which uses locally computed ranking functions to construct a global termination argument.

\noindent {\bf (3)} SCA is the natural abstract domain in connection with two program transformations -- {\em pathwise analysis} and {\em contextualization} -- that make imperative programs more amenable to bound analysis.
Pathwise analysis is used for reasoning about complete program paths, where inner loops are overapproximated by their transitive hulls.
Contextualization adds path-sensitivity to the analysis by checking which transitions can be executed subsequently.
Both transformations make use of the progress in SMT solver technology to reason about the long pieces of straight-line code given by program paths.
% The program transformations make the analysis more precise albeit at the cost of increasing program size:

%\noindent {\bf (3a)} {\em Pathwise analysis} is based on two ideas: First, to abstract not only single program statements or blocks but complete program paths. Second, to exploit the looping structure of programs by choosing paths from loop header back to header; these paths are the program entities on which we expect the linear change of individual norms to take place.
%%
%Thus, we enumerate all cycle-free paths from a location $\loc$ to $\loc$, insert the transitive hulls of the inner loops on all of these paths at the headers of the respective loops, and contract the transition relations on the resulting paths using SCA in order to derive a transition system.
%This has the advantage that we avoid computing intermediate predicates for detecting infeasible paths or size-change abstracting paths. \todo{M: was ist mit intermediate predicates gemeint?}

%\noindent {\bf (3b)} {\em Contextualization} enriches the state space by adding to every transition the information which transition is executed next; this makes it possible to detect transitions that cannot be executed subsequently.
%Our bound analysis then exploits the graph structure resulting from contextualization.
%Since pathwise analysis contracts large paths from $\loc$ to $\loc$ into single transitions, contextualization is particularly important after pathwise analysis.

%We can now put together all components to describe our approach:

\noindent{\em Summary of our Approach.}
To determine how often a location $\loc$ of program $\prog$ can be visited, we proceed in two steps akin to~\cite{conf/pldi/GulwaniZ10}: First, we compute a disjunctive transition system $\transinv$ for $\loc$ from $\prog$. Second, we use $\transinv$ to compute a bound on the number of visits to $\loc$. For the first step we recursively compute transition systems for nested loops and summarize them disjunctively by transitive hulls computed with SCA.
We enumerate all cycle-free paths from $\loc$ back to $\loc$, and derive a disjunctive transition system $\transinv$ from these paths and the summaries of the inner loops using \emph{pathwise analysis}.
For the second step we exploit the potential of SCA for automatic bound computation by first abstracting $\transinv$ using norms extracted from the program and then computing bounds solely on the abstraction. We use \emph{contextualization} to increase the precision of the bound computation.
Our method thus clearly addresses the challenges {\bf (A)} to {\bf (D)} discussed above. In particular, we make the following new contributions:

\begin{itemize}
\item We are the first to exploit SCA for bound analysis by using its ability of composing global bounds from bounds on locally extracted norms and disjunctive reasoning.
    Our technical contributions are the first algorithm for computing bounds with SCA (Algorithm~\ref{alg:computeBound}) and the disjunctive summarization of inner loops with SCA (Algorithm~\ref{alg:transitionSystem}).
\item We are the first to describe how to apply SCA on imperative programs.
Our technical contributions are two program transformations: pathwise analysis (Subsection~\ref{subsec:pathwise-analysis}), which exploits the looping structure of imperative programs, and contextualization (Subsection~\ref{subsec:contextualization}).
These program transformations make imperative programs amenable to bound analysis by SCA.
\item We obtain a competitive bound algorithm that captures the essential ideas of earlier termination and bound analyses in a simpler framework.
    Since bound analysis generalizes termination analysis, many of our methods are relevant for termination.
    Our experimental section shows that we can handle a large percentage of standard C programs.
    \final{We give a detailed comparison with related work on termination and bound analysis in the extended version of this paper available on the website of the first author.}
    \full{We give a detailed comparison with related work on termination and bound analysis in Section~\ref{sec:comparison}.}
\end{itemize}

% Our approach captures the essential ideas of previous work in a simpler framework and is effective in practice

%In Sec.~\ref{sec:related} and Appendix~\ref{sec:comparison} we give a detailed comparison with earlier work, most notably the {\sc Terminator} tool~\cite{conf/pldi/CookPR06}, and the more recent tools {\sc Loopfrog}~\cite{conf/cav/KroeningSTW10} and {\sc SPEED}~\cite{conf/pldi/GulwaniZ10}.
%We conclude that our bound analysis captures the essential ideas of these approaches in a simpler framework.
%In Section~\ref{sec:experiments}, we describe our experiments.
% and demonstrate that we can automatically compute bounds for a large %percentage of standard C programs.
%We conclude that our approach is not only theoretically simple and appealing, %but also works in practice.

% Our work will foster cross-fertilization between the imperative and functional world

% Room for refinement of our SCA approach for imperative programs: more complex program transformations such as~\cite{conf/pldi/GulwaniJK09} could be explored.

%\subsection{Contributions}

% Why SCA is a natural choice for termination and bound analysis
%We believe that every termination / bound analysis needs to contain the following elements:
%\begin{itemize}
%\item local progress measures (the iterators of for-loops, other counter variables)
%\item monotonic changes of the local progress measures (monotonic changes normally suffice)
%\item disjunction (needed for loops with phases, flags, etc.)
%\end{itemize}
%Because SCA consists exactly of the above identified minimal structure needed,
%SCA lies at the heart of the termination / bound problem.
%Our contributions are to identify SCA as the core for the analysis of imperative programs,
%and to give the first analysis of imperative program with SCA.


\nop{
% We explain our assumption/intuition on the structure of software programs
We will now discuss why we believe that SCA is the adequate abstract domain for bound analysis. Progress in most software depends on the linear change of integer-valued functions on the program state (e.g., counter variables, size of lists, height of trees, etc.), which we call \emph{norms}. \footnote{The importance of linear change is witnessed by the success of the abstract domains mentioned in (A) above.} Progress can normally be observed on paths from the start location of a loop back to this start location.
Therefore such paths are the right entity to extract norms and to be size-change abstracted.
The vast majority of non-linear bounds in real-life programs stems from two sources -- inner loops and loop phases -- and not from inherent non-linear behavior as in numeric algorithms. For most bounds, we can therefore
exploit the nesting structure of the loops, and compose them from bounds
on norms. Upper bounds for norms typically consist of easily established facts such as size comparisons between variables and can be computed by classical conjunctive domains.

\section{Move this to comparison section ?}


In~\cite{conf/cav/KroeningSTW10} Kroening et al. report that for most of the examples found in practice the full generality of the termination criterion underlying {\sc Terminator} and stated in~\cite{conf/lics/PodelskiR04} is not necessary.
We will show an interesting connection to the termination criterion of SCA.

The proof rules of the reachability-bound problem were ad hoc.
SCA generalizes all the proof rules stated in \cite{conf/pldi/GulwaniZ10} and is therefore strictly more general.
Moreover SCA offers an established framework in which these rules can be placed and offers a natural framework for further refinement.

As our implementation is closest to the {\sc SPEED} tool we state the following technical contributions:
\begin{itemize}
\item The enabledness check of {\sc SPEED} is flawed for more than two transitions and produces wrong results.
    With our SCA framework we correctly generalize the enabledness check to an arbitrary number of transitions.
%\item By borrowing the calling-context graph technique from the size-change literature we are able to handle loops that we could not be handled before.
\end{itemize}


Our experiments show that we can get a scalable solution:
\begin{itemize}
\item On C-code, whereas the experiments of the experiments of {\sc SPEED} were on .net code.
\item As the proposed approach is strictly more general - as we will demonstrate later - we can show that the methodology works on C-code and .net code found in practice.
\item Our experiments were executed on benchmarks from the WCET community as well as on cBench.
\end{itemize}

}



==> include/introduction.tex <==
\svnid{$Id$}
\section{Introduction}

%Structure:
%- what is the problem and why is it important
%- what are the difficulties in solving it
%- what is our solution
%- why does it solve the difficulties
%- how does it compare to the approaches from the literature


% introduction and importance of the bound problem

Computing symbolic bounds for the resource consumption of programs is an active area of research~\cite{conf/pldi/GulwaniZ10,conf/popl/GulwaniMC09,conf/pldi/GulwaniJK09,conf/esop/HoffmannH10,conf/popl/JostHLH10,conf/sigsoft/GoldsmithAW07,MH94} of great practical importance. Most questions about resource bounds can be reduced to bounds on program variables.
Our research is motivated by the following challenges:

%Since global ranking functions have to reflect the program structure they are typically lexicographic and quite complicated.
%For {\em resource bounds}, the natural method is to introduce a variable $k$ to log the resource consumption, and compute an upper bound on $k$ by an invariant generator.
%The construction principles for ranking functions and bounds are very similar.

% Challenges in bound computation (and termination)

\smallskip

\noindent{\bf (A)} Bounds are often {\em complex non-linear arithmetic expressions} built from $+,*,\max$ etc.
Therefore, abstract domains based on linear invariants (e.g.~intervals, octagons, polyhedra) are not directly applicable for bound computation.

\smallskip

\noindent{\bf (B)} The proof of a given bound often requires {\em disjunctive invariants} that can express loop exit conditions, phases, and flags which affect program behavior.
Although recent research made progress on computing disjunctive invariants~\cite{conf/pldi/GulwaniZ10,conf/pldi/GulwaniJK09,conf/lics/PodelskiR04,conf/pldi/CookPR06,conf/popl/BerdineCCDO07,conf/asian/PopeeaC06,Reps06}, this is still a challenging research topic.
Note that the domains mentioned in (A) are conjunctive.

\smallskip

\noindent{\bf (C)} It is {\em difficult to predict a bound in terms of a template} with parameters because (1) the search space for suitable bounds is huge, and
(2) the bound is a global property of the program and therefore a local analysis is not possible.

\smallskip

\noindent{\bf (D)} It is not clear how to {\em exploit the looping structure} for bound computation to achieve compositionality in the analysis.
This is in contrast to automatic termination analysis where the cutpoint technique~\cite{conf/pldi/CookPR06,conf/popl/BerdineCCDO07} is used standardly.
%In particular, the cutpoint technique~\cite{conf/pldi/CookPR06,conf/popl/BerdineCCDO07} which yields compositionality in termination proofs, is imprecise for bound
%computation, cf.~Sec.~\ref{subsec:example-abstraction}).

%Abstraction is the way that static analysis deals with undecidability.

% What is SCA
We believe that the size-change abstraction (SCA)~by Lee et al.~\cite{conf/popl/LeeJB01,mcs-integers} is the right abstract domain for addressing the above identified challenges.
SCA is a predicate abstraction domain that consists of (in)equality constraints between integer-valued variables and boolean combinations thereof in {\em disjunctive} normal form DNF.
The constraints can be separated into \emph{control predicates} which describe location invariants and \emph{transition predicates} which describe the monotonic change (increase, constant, or decrease) of the variables in one computation step.

% Why is SCA an attractive abstract domain
SCA is an attractive abstract domain for two reasons:
First, SCA is rich enough to capture the progress of many programs.
It has been successfully applied for automatic termination proofs of recursive functions in functional and declarative languages and is implemented in widely used systems such as ACL2~\cite{conf/cav/ManoliosV06}, Isabelle~\cite{conf/cade/Krauss07} etc. \todo{find some prolog citation}
Second, SCA is a simple abstraction that achieves a good trade-off between expressiveness and computational complexity.
For example, SCA termination is decidable and ranking functions can be extracted on terminating instances in PSPACE~\cite{mcs-integers}.
The simplicity of SCA sets it apart from other disjunctive abstract domains used for termination/bounds such as transition predicate abstraction~\cite{conf/popl/PodelskiR05} and powerset abstract domains~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07}.

% We explain our assumption/intuition on the structure of software programs
\todo{Sumit: Could be left out for lack of space}
We will now discuss why we believe that SCA is the adequate abstract domain for bound analysis. Progress in most software depends on the linear change of integer-valued functions on the program state (e.g., counter variables, size of lists, height of trees, etc.), which we call \emph{norms}. \footnote{The importance of linear change is witnessed by the success of the abstract domains mentioned in (A) above.} Progress can normally be observed on paths from the start location of a loop back to this start location.
Therefore such paths are the right entity to extract norms and to be size-change abstracted.
The vast majority of non-linear bounds in real-life programs stems from two sources -- inner loops and loop phases -- and not from inherent non-linear behavior as in numeric algorithms. For most bounds, we can therefore
exploit the nesting structure of the loops, and compose them from bounds
on norms. Upper bounds for norms typically consist of easily established facts such as size comparisons between variables and can be computed by classical conjunctive domains.

\todo{Above paragraph unclear. Why do we in the middle of the argument mention start-to-end paths ? Where do we say why SCA is important as promised ?}

%Our approach to bound computation follows recent approaches from the literature for exploiting the structure of loops.

% SCA has interesting properties that we use in our analysis

\paragraph{Three crucial features of SCA.}
Our analysis uses three crucial features of SCA:

\noindent (1) Disjunctive transitive hulls can be easily computed in SCA, because SCA is a finite abstract domain.
These transitive hulls have the crucial property to preserve termination.
We will make use of the capability of SCA to compute transitive hulls for summarizing inner loops.

\noindent (2) SCA offers a framework for separating control invariants from transition invariants. Thus, the termination / bounds analysis only needs to operate on the transition invariants. This greatly simplifies the problem of bound computation. To achieve this separation we propose to apply program transformations which encode program behavior into the control locations {\em before} the bounds analysis. Our transformations may enlarge the number of control locations but will increase the precision of a subsequent bound computation. We present two program transformations -- \emph{pathwise analysis} and \emph{contextualization} -- which achieve
 this separation and strengthen the subsequent bound algorithm.

\noindent (3) SCA separates the actual computation of a bound from finding
the right template for the bound. As argued in {\bf (C)} above,
this is an important step in an automatic bound analysis. SCA achieves this separation as follows: We only consider small program parts for extracting norms. After the extraction we consider only the abstracted program for bound computation. At this point we already know how the (global) bound can be
expressed in terms of the (local) norms. A similar separation of concerns has been successfully used for automatic termination analysis in the {\sc Terminator} tool~\cite{conf/pldi/CookPR06} which uses locally computed ranking functions to construct a global termination argument.


% How our solution looks like

\paragraph{Our approach}
investigates how often a particular location $\loc$ of a program $\prog$ can be visited. Following earlier work~\cite{conf/pldi/GulwaniZ10}, we proceed in two steps: First, we compute a disjunctive transition system $\transinv$ for $\loc$ from $\prog$. Second, we use $\transinv$ to compute a bound on the number of visits to $\loc$. For the first step we recursively compute transition systems for inner loops and summarize them disjunctively by transitive hulls computed with SCA.
We enumerate all cycle-free paths from $\loc$ back to $\loc$, and derive a disjunctive transition system $\transinv$ from these paths and the summaries of the inner loops using the program transformation \emph{pathwise analysis} described below. For the second step we exploit the potential of SCA for automatic bound computation as explained above by first abstracting $\transinv$ using norms extracted from the program and then computing bounds solely on the abstraction. We use the program transformation \emph{contextualization} described below to increase the precision of the bound computation.

We will now describe the two program transformations we use:

{\em Pathwise analysis} is based on two ideas: First, to analyze not only single program statements or blocks but complete program paths. Second, to exploit the looping structure of programs by choosing paths from loop header back to header; these paths are the program entities on which we expect the linear change of norms to take place.
%
Technically, pathwise analysis enumerates all cycle-free paths from a location $\loc$ to $\loc$, inserts the transitive hulls of the inner loops on all of these paths at the header of the respective loops, and contracts the transition relations on the resulting paths in order to derive a transition system. This has the advantage that we avoid computing intermediate predicates for detecting infeasible paths or size-change abstracting paths. Thus, we separate control from transition invariants.

{\em Contextualization} is adding the information which transition is executed next to every control location; this makes it possible to detect transitions that cannot be executed subsequently. In particular, we refine the control flow graph by deleting infeasible edges; this benefits the subsequent bound analysis, which exploits the SCC component graph of CFGs. Our refinement separates control from transition invariants, because it avoids the explicit computation of pre- and postconditions of transitions which would be needed for reasoning about the potential interleavings of transitions in the bound computation.

Both transformations make use of the progress in SMT solver technology to reason about the long pieces of straight-line code given by program paths.

% Our methodology answers the challenges
\todo{Sumit: Discussion of this paragraph should come in the technical section to save space, Florian: I leave it here for now as a todo list}
Our methodology solves the above challenges (A)-(D) as follows:
For {\bf (A)}, we compute global invariants with standard linear abstract domains.
Upper bounds on norms can usually be established by these invariants.
For {\bf (B)}, we use SCA to compute disjunctive summaries of inner loops.
We compute disjunctive transition systems by enumerating cycle-free paths and contracting the transition relations of these paths;
For {\bf (C)}, we extract norms from paths that start from loop headers and go back to the headers.
Our experiments (and also those of~\cite{conf/pldi/GulwaniZ10,conf/pldi/CookPR06}) confirm that these paths have the right granularity to extract norms.
Our bound algorithm then composes complex bounds from bounds on norms using $+,*,\max$.
For {\bf (D)}, our pathwise-analysis exploits the looping structure of imperative programs.
In contrast to the cutpoints method it retains enough information to compute precise bounds.

% Our approach captures the essential ideas of previous work in a simpler framework and is effective in practice
In Section~\ref{sec:comparison}, we give a detailed comparison with earlier approaches on the termination and bound problem.
Most notably, these approaches include the {\sc Terminator} tool~\cite{conf/pldi/CookPR06}, and the more recent tools {\sc Loopfrog}~\cite{conf/cav/KroeningSTW10} and {\sc SPEED}~\cite{conf/pldi/GulwaniZ10}.
We conclude from our comparison that our bound analysis captures the essential ideas of these approaches in a simpler framework.
In Section~\ref{sec:experiments}, we describe our experiments and demonstrate that we can automatically compute bounds for a large percentage of standard C programs.
We conclude that our approach is not only theoretically simple and appealing, but also works in practice.

% Our work will foster cross-fertilization between the imperative and functional world
Up to the present date research on the termination/bound problem has been divided into separate lines for the imperative and functional/declarative world.
Our work for the first time bridges this gap by using SCA, which has been developed for functional programs, in an imperative setting.
We hope that this will foster the transfer of ideas and techniques between these two lines of research.
We give the first example of such a cross-fertilization by using the program transformation contextualization taken from work on functional programs~\cite{conf/cav/ManoliosV06}.


% Room for refinement of our SCA approach for imperative programs.
\todo{Move to conclusion?}
We believe that identifying SCA as the right abstract domain for bound analysis of imperative programs is a main contribution of this paper.
We view our solution as one choice in the solution space offered by this powerful abstraction framework.
Further investigations on SCA are worthwhile, for example, our bound algorithm is a simple greedy algorithm, which handles many programs occurring in practice, but which does not exploit the full power of SCA.
%; more complex program transformations such as~\cite{conf/pldi/GulwaniJK09} could be explored.

\subsection{Contributions}

% Why SCA is a natural choice for termination and bound analysis
%We believe that every termination / bound analysis needs to contain the following elements:
%\begin{itemize}
%\item local progress measures (the iterators of for-loops, other counter variables)
%\item monotonic changes of the local progress measures (monotonic changes normally suffice)
%\item disjunction (needed for loops with phases, flags, etc.)
%\end{itemize}
%Because SCA consists exactly of the above identified minimal structure needed,
%SCA lies at the heart of the termination / bound problem.
%Our contributions are to identify SCA as the core for the analysis of imperative programs,
%and to give the first analysis of imperative program with SCA.

\begin{itemize}
\item We give the first algorithm for abstracting imperative programs with SCA.
Our technical contributions are the summarization of inner loops with SCA and the pathwise-analysis, which makes SCA sufficiently precise.
\item We are the first to exploit the separation between control and transition invariants resulting from SCA for bound analysis.
Our technical contributions are the first algorithm for computing bounds from size-change programs and the use of the program transformation contextualization for bound computation, which makes bound computation sufficiently precise.
\item We obtain a competitive bound algorithm with simpler concepts than bound algorithms from the literature.
    We give a qualitative comparison with other approaches in our related work section.
    Our experimental section shows that we can handle a large percentage of standard C programs.
\end{itemize}

\nop{
% We explain our assumption/intuition on the structure of software programs
We will now discuss why we believe that SCA is the adequate abstract domain for bound analysis. Progress in most software depends on the linear change of integer-valued functions on the program state (e.g., counter variables, size of lists, height of trees, etc.), which we call \emph{norms}. \footnote{The importance of linear change is witnessed by the success of the abstract domains mentioned in (A) above.} Progress can normally be observed on paths from the start location of a loop back to this start location.
Therefore such paths are the right entity to extract norms and to be size-change abstracted.
The vast majority of non-linear bounds in real-life programs stems from two sources -- inner loops and loop phases -- and not from inherent non-linear behavior as in numeric algorithms. For most bounds, we can therefore
exploit the nesting structure of the loops, and compose them from bounds
on norms. Upper bounds for norms typically consist of easily established facts such as size comparisons between variables and can be computed by classical conjunctive domains.

\section{Move this to comparison section ?}

In~\cite{conf/cav/KroeningSTW10} Kroening et al. report that for most of the examples found in practice the full generality of the termination criterion underlying {\sc Terminator} and stated in~\cite{conf/lics/PodelskiR04} is not necessary.
We will show an interesting connection to the termination criterion of SCA.

The proof rules of the reachability-bound problem were ad hoc.
SCA generalizes all the proof rules stated in \cite{conf/pldi/GulwaniZ10} and is therefore strictly more general.
Moreover SCA offers an established framework in which these rules can be placed and offers a natural framework for further refinement.

As our implementation is closest to the {\sc SPEED} tool we state the following technical contributions:
\begin{itemize}
\item The enabledness check of {\sc SPEED} is flawed for more than two transitions and produces wrong results.
    With our SCA framework we correctly generalize the enabledness check to an arbitrary number of transitions.
%\item By borrowing the calling-context graph technique from the size-change literature we are able to handle loops that we could not be handled before.
\end{itemize}


Our experiments show that we can get a scalable solution:
\begin{itemize}
\item On C-code, whereas the experiments of the experiments of {\sc SPEED} were on .net code.
\item As the proposed approach is strictly more general - as we will demonstrate later - we can show that the methodology works on C-code and .net code found in practice.
\item Our experiments were executed on benchmarks from the WCET community as well as on cBench.
\end{itemize}

}



==> include/macros.tex <==
\svnid{$Id$}

\newcounter{counter}
%\newtheorem{definition}[counter]{Definition}
%\newtheorem{theorem}[counter]{Theorem}
%\newtheorem{lemma}[counter]{Lemma}
%\newtheorem{corollary}[counter]{Corollary}
%\newtheorem{proposition}[counter]{Proposition}
%\newtheorem{property}[counter]{Property}
%\newtheorem{claim}[counter]{Claim}
%\newtheorem{observation}[counter]{Observation}
%\newtheorem{remark}[counter]{Remark}
%\newtheorem{example}[counter]{Example}
%\newtheorem{fact}[counter]{Fact}

\newcommand{\cutpoint}{\ensuremath{c}}
\newcommand{\cutpoints}{\ensuremath{C}}

%sets and relations
\newcommand{\element}{\ensuremath{e}}
\newcommand{\set}{\ensuremath{A}}
\newcommand{\relation}{\ensuremath{B}}
\newcommand{\relationset}{\ensuremath{\mathcal{C}}}

%set of variables
\newcommand{\varset}{\ensuremath{X}}
\newcommand{\varsetP}{\ensuremath{X^\prime}}
\newcommand{\oc}{\ensuremath{o}}
\newcommand{\ocs}{\ensuremath{O}}

\newcommand{\countvar}{\ensuremath{n}}
\newcommand{\val}{\ensuremath{\mathit{Val}}}

%program
\newcommand{\prog}{\ensuremath{P}}
\newcommand{\vars}{\ensuremath{\mathit{Var}}}
\newcommand{\varsP}{\ensuremath{\vars^\prime}}
\newcommand{\varsPP}{\ensuremath{\vars^{\prime\prime}}}
\newcommand{\loc}{\ensuremath{l}}
\newcommand{\locs}{\ensuremath{L}}
\newcommand{\edges}{\ensuremath{E}}
\newcommand{\transfct}{\ensuremath{\mathit{stmt}}}
\newcommand{\locstart}{\ensuremath{\loc_{\mathit{start}}}}
\newcommand{\locend}{\ensuremath{\loc_{\mathit{end}}}}
\newcommand{\state}{\ensuremath{s}}
\newcommand{\states}{\ensuremath{\Sigma}}
\newcommand{\trn}{\ensuremath{\rho}}
\newcommand{\trns}{\ensuremath{\Gamma}}
\newcommand{\norm}{\ensuremath{n}}
\newcommand{\norms}{\ensuremath{N}}
\newcommand{\normsP}{\ensuremath{\norms^\prime}}
\newcommand{\paath}{\ensuremath{\pi}}
\newcommand{\paths}{\ensuremath{\mathtt{paths}}}
\newcommand{\rundag}{\ensuremath{\mathcal{G}}}
\newcommand{\looop}{\ensuremath{\mathit{loop}}}

\newcommand{\assign}{\ensuremath{\mathit{Assign}}}
\newcommand{\assume}{\ensuremath{\mathit{Assume}}}

\newcommand{\Summary}{\ensuremath{\mathsf{summary}}}
\newcommand{\ITE}{\ensuremath{\mathtt{ITE}}}
\newcommand{\rel}{\ensuremath{\mathtt{rel}}}
\newcommand{\contract}{\ensuremath{\mathtt{rel}}}
\newcommand{\header}{\ensuremath{\mathit{header}}}
\newcommand{\closure}{\ensuremath{\mathit{hull}}}
\newcommand{\IsHeader}{\ensuremath{\mathtt{IsHeader}}}

%size-change program
%\newcommand{\scvars}{{\ensuremath{SCV}}}
%\newcommand{\scvarsP}{\ensuremath{\scvars^\prime}}
%\newcommand{\scvarsPP}{\ensuremath{\scvars^{\prime\prime}}}
%\newcommand{\scloc}{\ensuremath{f}}
%\newcommand{\sclocs}{\ensuremath{\Lambda}}
%\newcommand{\scedges}{\ensuremath{\Delta}}

\newcommand{\mc}{\ensuremath{c}}
\newcommand{\mcs}{\ensuremath{\mathit{MCs}}}
\newcommand{\scr}{\ensuremath{T}}
\newcommand{\scrs}{\ensuremath{\mathit{SCRs}}}
\newcommand{\scrset}{\ensuremath{\mathcal{S}}}

%abstraction
\newcommand{\transinv}{\ensuremath{\mathcal{T}}}
\newcommand{\pred}{\ensuremath{p}}
\newcommand{\preds}{\ensuremath{P}}
\newcommand{\predset}{\ensuremath{\mathcal{P}}}
\newcommand{\predtran}{\ensuremath{q}}
\newcommand{\predtrans}{\ensuremath{Q}}
\newcommand{\predtranset}{\ensuremath{\mathcal{Q}}}

\newcommand{\nop}[1]{}

\newcommand{\SCCs}{\ensuremath{\mathit{SCCs}}}
\newcommand{\SCC}{\ensuremath{\mathit{SCC}}}
\newcommand{\bound}{\ensuremath{\mathit{b}}}
\newcommand{\sccBnds}{\ensuremath{\mathit{SCCsOnLevelBnds}}}
\newcommand{\SCCsOnLevel}{\ensuremath{\mathit{SCCsOnLevel}}}

\newcommand{\TransSys}{\mathtt{TransSys}}
%\newcommand{\TransHull}{\mathtt{TransHull}}
\newcommand{\Contextualize}{\mathtt{Contextualize}}
\newcommand{\ComputeBound}{\mathtt{Bound}}
\newcommand{\ComputeBoundSCC}{\mathtt{BndSCC}}

\newcommand{\NonIncr}{\ensuremath{\mathit{NonIncr}}}
\newcommand{\DecrBnded}{\ensuremath{\mathit{DecrBnded}}}
\newcommand{\BndedEdgs}{\ensuremath{\mathit{BndedEdgs}}}

\newcommand{\hv}[1]{\quad\\[1ex]\fbox{\begin{minipage}{9cm}{\em #1}\end{minipage}}}
\newcommand{\todo}[1]{$\star$\marginpar{\textbf{TODO:} #1}}
\newcommand{\changed}[1]{{\color{red} #1}} 

==> include/model.tex <==
\svnid{$Id$}

\vspace{-0.2cm}

\section{Program Model and Size-change Abstraction}
\label{sec:model}

\vspace{-0.2cm}

%In this section we introduce our program model and the size-change %abstraction.
%At the same time we give the definitions and notations necessary for the %presentation of our analysis algorithms in Sections~\ref{sec:abstraction} %and~\ref{sec:bound-computation}.

\paragraph{\bfseries Sets and Relations.} Let $\set$ be a set.
The concatenation of two relations $\relation_1,\relation_2 \in 2^{\set \times \set}$ is the relation $\relation_1 \circ \relation_2 = \{(\element_1,\element_3) \mid \exists \element_2. (\element_1,\element_2) \in \relation_1 \wedge (\element_2,\element_3) \in \relation_2 \}$.
$Id = \{(\element,\element) \mid \element \in \set\}$ is the \emph{identity relation} over $\set$.
Let $\relation \in 2^{\set \times \set}$ be a relation.
%The \emph{transitive hull} $\relation^+ \in 2^{\set \times \set}$ is the least relation with $\relation \subseteq \relation^+$ and $\relation^+ \circ \relation \subseteq \relation^+$.
%The \emph{reflexive transitive hull} $\relation^* \in 2^{\set \times \set}$ is the least relation with $\relation \subseteq \relation^*$ and $\relation^* \circ \relation \subseteq \relation^*$.
We inductively define the $k$-\emph{fold} \emph{exponentiation} of $\relation$ by $\relation^k = \relation^{k-1} \circ \relation$ and $\relation^0 = Id$.
$\relation^+ = \bigcup_{k \ge 1} \relation^k$ resp. $\relation^* = \bigcup_{k \ge 0} \relation^k$ is the \emph{transitive}- resp. \emph{reflexive transitive hull} of $\relation$.
We lift the concatenation operator $\circ$ to sets of relations by defining $\relationset_1 \circ \relationset_2 = \{\relation_1 \circ \relation_2 \mid \relation_1 \in \relationset_1, \relation_2 \in \relationset_2\}$ for sets of relations $\relationset_1,\relationset_2 \subseteq 2^{\set \times \set}$.
We set $\relationset^0 = \{Id\}$; $\relationset^k, \relationset^+$ etc. are defined analogously.

%Let $\relationset \subseteq 2^{\set \times \set}$ be a relation.
%We inductively define the $k$-\emph{fold} \emph{exponentiation} of %$\relationset$ by $\relationset^k = \relationset^{k-1} \circ \relationset$ and %$\relationset^0 = \{Id\}$.
%$\relationset^+ = \bigcup_{k \ge 1} \relationset^k$ resp. $\relationset^* = %\bigcup_{k \ge 0} \relationset^k$ is the \emph{transitive}-resp. %\emph{reflexive transitive hull} of $\relationset$.

%\subsection{Program Model}
\paragraph{\bfseries Program Model.}
We introduce a simple program model for sequential imperative programs without procedures.
Our definition models explicitly the essential features of imperative programs, namely branching and looping. In Section~\ref{sec:abstraction} we will explain how to exploit the graph structure of programs in our analysis algorithm.
We leave the extension to concurrent and recursive programs for future work.

\begin{definition}[Transition Relations / Invariants] %$\{$ Relation $|$ Set $|$ System $|$ Invariant $\}$
\label{def:program}
  Let $\states$ be a set of \emph{states}.
  The set of \emph{transition relations} $\trns = 2^{\states \times \states}$ is the set of relations over $\states$.
%  We use the usual set operator $\circ$ to concatenate transition relations, i.e., for all $\trn_1,\trn_2 \in \trns$ we have $\trn_1 \circ \trn_2 = \{(\state_1,\state_3) \mid \exists \state_2. (\state_1,\state_2) \in \trn_1 \wedge (\state_2,\state_3) \in \trn_2 \}$, and to define the usual
%  $\trn^+ = \bigcup_{k \ge 1} \trn^k$ and $\trn^* = \bigcup_{k \ge 0} \trn^k$ are the transitive
  A \emph{transition set} $\transinv \subseteq \trns$ is a finite set of transition relations.
%  We lift the operator $\circ$ to transition sets by setting $\transinv_1 \circ \transinv_2 = \{\trn_1 \circ \trn_2 \mid \trn_1 \in \transinv_1, \trn_2 \in \transinv_2\}$ for transition sets $\transinv_1,\transinv_2$.
  %In a formula involving sets $\transinv$ stands for the transition relation $\bigcup \transinv$.
  Let $\trn \in \trns$ be a transition relation.
  $\transinv$ is a \emph{transition system} for $\trn$, if $\trn \subseteq \bigcup \transinv$.
  $\transinv$ is a \emph{transition invariant} for $\trn$, if $\trn^* \subseteq \bigcup \transinv$.
\end{definition}

%\begin{lemma}
%  $\bigcup \transinv^* = (\bigcup \transinv)^*$.
%\end{lemma}
%\begin{proof}
%\begin{displaymath}
%  \bigcup \transinv^* = \bigcup \bigcup_{k \ge 0} \transinv^k = \bigcup_{k \ge 0} \bigcup \transinv^k = \bigcup_{k \ge 0} (\bigcup \transinv)^k = (\bigcup \transinv)^*.
%\end{displaymath}
%\end{proof}

\begin{definition}[Program, Path, Trace, Termination]
  A \emph{program} is a tuple $\prog = (\locs, \edges)$, where $\locs$ is a finite set of \emph{locations}, and $\edges \subseteq \locs \times \trns \times \locs$ is a finite set of \emph{transitions}. We write $\loc_1 \xrightarrow{\trn} \loc_2$ to denote a transition $(\loc_1,\trn,\loc_2)$.

  A \emph{path} of $\prog$ is a sequence $\loc_0 \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \cdots$ with $\loc_i \xrightarrow{\trn_i} \loc_{i+1} \in \edges$ for all $i$.
  Let $\paath = \loc_0 \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \loc_2 \cdots \loc_k \xrightarrow{\trn_k} \loc_{k + 1}$ be a finite path.
  $\paath$ is \emph{cycle-free}, if $\paath$ does not visit a location twice except for the end location, i.e., $\loc_i \neq \loc_j$ for all $0 \le i < j \le k$.
  The \emph{contraction} of $\paath$ is the transition relation $\rel(\paath) = \trn_0 \circ \trn_1 \circ \cdots \circ \trn_k$ obtained from concatenating all transition relations along $\paath$.
  Given a location $\loc$, $\mathtt{paths}(\prog,\loc)$ is the set of all finite paths with start and end location $\loc$.
  A path $\paath \in \mathtt{paths}(\prog,\loc)$ is \emph{simple}, if all locations, except for the start and end location, are different from $\loc$.

  %$\mathtt{paths}(\prog,\loc)$ is the set of all paths $\loc \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \loc_2 \cdots \loc_k \xrightarrow{\trn_k} \loc$ of $\prog$ that have the start and end location $\loc$.

  A \emph{trace} of $\prog$ is a sequence $(\loc_0,\state_0) \xrightarrow{\trn_0} (\loc_1,\state_1) \xrightarrow{\trn_1} \cdots$ such that $\loc_0 \xrightarrow{\trn_0} \loc_1 \xrightarrow{\trn_1} \cdots$ is a path of $\prog$, $\state_i \in \states$ and $(\state_i,\state_{i+1}) \in \trn_i$ for all $i$.
  $\prog$ is \emph{terminating}, if there is no infinite trace of $\prog$.
\end{definition}

Note that a cycle-free path $\paath \in \mathtt{paths}(\prog,\loc)$ is always simple.
%Further note that our definition of programs allows to model branching and looping precisely and naturally:
%imperative programs can usually be represented as CFGs whose edges are labeled with assign and assume statements as can be seen on Example~\ref{ex:abstraction}
Further note that our definition of programs allows to model branching and looping precisely and naturally: imperative programs can usually be represented as CFGs whose edges are labeled with assign and assume statements.

\begin{definition}[Transition Relation of a Location] %
  Let $\prog = (\locs,\edges)$ be a program and $\loc \in \locs$ a location.
  The \emph{transition relation of} $\loc$ is the set
  $\prog|_\loc = \bigcup_{\text{simple } \paath \in \mathtt{paths}(\prog,\loc)}\rel(\paath)$.

%  The \emph{transition relation} $\prog|_\loc$ \emph{of} $\loc$ of $\prog$ w.r.t. $\loc$ is the set of all pairs of states $(\state_a,\state_b)$ s.t. there exists a trace of $\prog$ that reaches $(\loc,\state_a)$ and later $(\loc,\state_b)$ but that does not come by location $\loc$ in between.
%  Formally, $\prog|_\loc = \{ (\state_a,\state_b) \mid \text{there is a trace } (\loc_0,\state_0) \xrightarrow{\trn_0} (\loc_1,\state_1) \xrightarrow{\trn_1} \ldots \text{ of } \prog \text{ with } \ \loc_i = \loc_j = \loc, \state_i = \state_a, \state_j = \state_b,  i < j \text{ and } \forall i < k < j. \loc_k \neq \loc \}$.
\end{definition}

\subsection{Order Constraints}
%
Let $\varset$ be a set of variables.
Given a variable $x$ we denote by $x^\prime$ its \emph{primed} version.
% and by $ x^{(i)}$ its version with $i$-primes.
We denote by $\varsetP$ the set $\{ x^\prime \ | \ x \in \varset\}$ of the primed variables of $\varset$.
We denote by $\rhd$ any element from $\{>,\ge\}$.

\begin{definition}[Order Constraint]
  An \emph{order constraint} over $\varset$ is an inequality $x \rhd y$ with $x,y \in \varset$.
\end{definition}

\begin{definition} [Valuation]
  The set of all \emph{valuations} of $\varset$ is the set $\val_\varset = \varset \rightarrow \mathbb{Z}$ of all functions from $\varset$ to the integers.
%
  Given a valuation $\sigma \in \val_\varset$ we define its \emph{primed valuation} as the function $\sigma^\prime \in \val_{\varset^\prime}$ with $\sigma^\prime(x^\prime) = \sigma(x)$ for all $x \in \varset$.
%
  Given two valuations $\sigma_1 \in \val_{\varset_1}, \sigma_2 \in \val_{\varset_2}$ with $\varset_1 \cap \varset_2 = \emptyset$ we define their \emph{union} $\sigma_1 \cup \sigma_2 \in \val_{\varset_1 \cup \varset_2}$ by
  $(\sigma_1 \cup \sigma_2)(x) = \left\{\begin{array}{ll}
        \sigma_1(x) & \text{  for } x \in X_1,\\
        \sigma_2(x) & \text{  for } x \in X_2.
  \end{array}\right.$
  %with $(\sigma_1 \cup \sigma_2)(x) = \sigma_1(x)$ for $x \in \varset_1$ and %$(\sigma_1 \cup \sigma_2)(x) = \sigma_2(x)$ for $x \in \varset_2$.
\end{definition}

\begin{definition} [Semantics]
  We define a \emph{semantic relation} $\models$ as follows:
  Let $\sigma \in \val_\varset$ be a valuation.
  Given an order constraint $x_1 \rhd x_2$ over $\varset$, $\sigma \models x_1 \rhd x_2$ holds, if $\sigma(x_1) \rhd \sigma(x_2)$ holds in the structure of the integers $(\mathbb{Z},\ge)$.
  Given a set $\ocs$ of order constraints over $\varset$, $\sigma \models \ocs$ holds, if $\sigma \models \oc$ holds for all $\oc \in \ocs$.
\end{definition}

\subsection{Size-change Abstraction (SCA)}
\label{subsec:scs}

We are using integer-valued functions on the program states to measure progress of a program. Such functions are called norms in the literature. Norms provide us sizes of states that we can compare.
We will use norms for abstracting programs.

\begin{definition}[Norm]
  A \emph{norm} $\norm \in \states \rightarrow \mathbb{Z}$ is a function that maps the states to the integers.
\end{definition}

% and to define bounds.

%\TODO{define bounds in terms of norms}
%\begin{definition}[Bound]
%  Let $\prog$ be a program and let $\norms$ be a set of norms of $\prog$.
%  A \emph{bound} is an arithmetic expression $e: \States \rightarrow \mathbb{Z}$ built from norms of $\norms$ such that there is no trace $(\loc_0,\state_0) \xrightarrow{\trn_0} (\loc_1,\state_1) \xrightarrow{\trn_1} (\loc_n,\state_n)$ with $n > e(\state_0)$.
%\end{definition}

We fix a finite set of norms $\norms$ for the rest of this subsection, and describe in Section~\ref{sec:heuristics} how to extract norms from programs automatically.
Given a state $\state \in \states$ we define a valuation $\sigma_\state \in \val_\norms$ by setting $\sigma_\state(\norm) = \norm(\state)$.

We will now introduce SCA.
Our terminology diverts from the seminal papers on SCA~\cite{conf/popl/LeeJB01,mcs-integers} because we focus on a logical rather than a graph-theoretic representation. The set of norms $\norms$ corresponds to the SCA ``variables'' in \cite{conf/popl/LeeJB01,mcs-integers}.

\begin{definition}[Monotonicity Constraint, Size-change Relation / Set, Concretization]
  The set of \emph{monotonicity constraints} $\mcs$ is the set of all order constraints over $\norms \cup \normsP$.
  The set of \emph{size-change relations} (SCRs) $\scrs = 2^\mcs$ is the powerset of $\mcs$.
  An \emph{SCR set} $\scrset \subseteq \scrs$ is a set of SCRs.
  We use the \emph{concretization function} $\gamma: \scrs \rightarrow \trns$ to map an SCR $\scr \in \scrs$ to a transition relation $\gamma(\scr)$ by defining $\gamma(\scr) = \{(\state_1,\state_2) \in \states \times \states \mid \sigma_{\state_1} \cup \sigma_{\state_2}^\prime \models \scr\}$ as the set of all pairs of states such that the evaluation of the norms on these states satisfy all the constraints of $\scr$.
  We lift the concretization function to SCR sets by setting $\gamma(\scrset) = \{\gamma(\scr) \mid \scr \in \scrset\}$ for an SCR set $\scrset$.
\end{definition}

%We have $\gamma(\scr_1 \cup \scr_2) = \gamma(\scr_1) \cap \gamma(\scr_2)$ because of
%\begin{displaymath}
%(\state_1,\state_2) \in \gamma(\scr_1 \cup \scr_2) \Leftrightarrow
%\forall \mc \in \scr_1 \cup \scr_2. (\state_1,\state_2) \models \mc \Leftrightarrow
%\forall \mc \in \scr_1. (\state_1,\state_2) \models \mc \wedge \forall \mc \in \scr_2. (\state_1,\state_2) \models \mc \Leftrightarrow
%(\state_1,\state_2) \in \gamma(\scr_1) \cap \gamma(\scr_1).
%\end{displaymath}
%Thus $\gamma$ is preservers finite meets.

Note that the abstract domain of SCRs has only finitely many elements, namely $3^{(2|\norms|)^2}$.
Further note that an SCR set corresponds to a formula in DNF.
%Thus every meet over an arbitrary number of elements yields the same results as the meet over some finite subset of the elements, formally,
%given a family of SCRs $\scrs^I$ there is a finite subset $J \subseteq I$ such that $\bigsqcap_{i \in I} \scr_i = \bigsqcap_{i \in J} \scr_i$.
%Therefore $\gamma$ preservers arbitrary meets.
%Thus, there exists a best abstraction function for transition relations. \hv{add reference, e.g. Cousot}

\begin{definition}[Abstraction Function]
  The \emph{abstraction function} $\alpha: \trns \rightarrow \scrs$ takes a transition relation $\trn \in \trns$ and returns the greatest SCR containing it, namely $\alpha(\trn) = \{\mc \in \mcs \mid \trn \subseteq \gamma(\mc)\}$.
  We lift the abstraction function to transition sets by setting $\alpha(\transinv) = \{\alpha(\trn) \mid \trn \in \transinv\}$ for a transition set $\transinv$.
\end{definition}

%Note that the equality $\bigcup \{\scr \in \scrs \mid \trn \subseteq \gamma(\scr)\} = \{\mc \in \mcs \mid \trn \models \mc\}$\todo{M: $\trn \models \mc$ ist nicht definiert} is a simple observation from the definitions, and that $\alpha$ is a best abstraction function.

%We have $\gamma(\alpha(\trn)) \subseteq \trn$ by $\gamma(\alpha(\trn)) = \gamma(\bigcup \{\scr \in \scrs \mid \trn \subseteq \gamma(\scr)\}) = \bigcap \{ \gamma(\scr) \mid \scr \in \scrs \wedge \trn \subseteq \gamma(\scr)\} \subseteq \trn$, which holds because $\gamma$ preserves arbitrary meets.
%
%We have $\alpha(\gamma(\scr)) = \bigcup \{\scr^\prime \in \scrs \mid \gamma(\scr) \subseteq \gamma(\scr^\prime)\} \sqsubseteq \scr$ by the definition of $\alpha$.
%
%Therefore $(\gamma,\alpha)$ are a Galois connection between the posets $(\scrs,\supseteq)$ and $(\trns,\subseteq)$, and we have
%$\gamma(\scr) \subseteq \trn \Leftrightarrow \scr \sqsubseteq \alpha(\trn)$,
%where $\gamma$ is the lower adjoint of $\alpha$ and $\alpha$ is the upper adjoint of $\gamma$.


\paragraph{Implementation of the abstraction.} $\alpha$ can be implemented by an SMT solver under the assumption that the norms are provided as expressions and that the transition relation is given as a formula such that the order constraints between these expressions and the formula fall into a logic that the SMT solver can decide.
%for every monotonicity constraint between norms the SMT solver can discharge %the query whether it is implied be the transition formula or not.

Using abstraction and concretization we can define concatenation of SCRs:
\begin{definition}[Concatenation of SCRs]
\label{def:transitive-hull}
  Given two SCRs $\scr_1, \scr_2 \in \scrs$, we define $\scr_1 \circ \scr_2$ to be the SCR $\alpha(\gamma(\scr_1) \circ \gamma(\scr_2))$.
  We lift the concatenation operator $\circ$ to SCR sets by defining $\scrset_1 \circ \scrset_2 = \{\scr_1 \circ \scr_2 \mid \scr_1 \in \scrset_1, \scr_2 \in \scrset_2\}$ for SCR sets $\scrset_1,\scrset_2 \in 2^{\scrs}$. $\scrset^0 = \{Id\}, \scrset^k, \scrset^+, \scrset^*$ etc. are defined in the natural way.

%  Let $\scrset$ be an SCR set.
%  We inductively define the $k$-\emph{fold} \emph{exponentiation} of $\scrset$ %by $\scrset^k = \scrset^{k-1} \circ \scrset$ and $\scrset^0 = \{Id\}$.
%  $\scrset^+ = \bigcup_{k \ge 1} \scrset^k$ resp. $\scrset^* = \bigcup_{k \ge %0} \scrset^k$ is the \emph{transitive}-resp. \emph{reflexive transitive hull} of $\scrset$.
\end{definition}

Concatenation of SCRs is conservative by definition, i.e., $\gamma(\scr_1 \circ \scr_2) \supseteq \gamma(\scr_1) \circ \gamma(\scr_2)$ and associative because of the transitivity of order relations.
Concatenation of SCRs can be effectively computed by a modified all-pairs-shortest-path algorithm (taking order relations as weights).
%
%Given an SCR set, we are interested in computing its transitive hull.
%
%\begin{definition}[Transitive Hull]
%\label
%  Let $\scrset$ be an SCR set.
%  The \emph{transitive hull} $\scrset^+$ of $\scrset$ is the least SCR set with $\scrset \subseteq \scrset^+$ and
%  $\scr_1 \circ \scr_2 \in \scrset^+$ for all $\scr_1,\scr_2 \in \scrset^+$.
%\end{definition}
%
Because the number of SCRs is finite, the transitive hull is computable.

The following theorem can be directly shown from the definitions. We will use it to summarize the transitive hull of loops disjunctively, cf.~Section~\ref{sec:abstraction}.

\begin{theorem}[Soundness]
\label{thm:soundness}
  Let $\trn$ be a transition relation and $\transinv$ a transition system for $\trn$.
  Then $\gamma(\alpha(\transinv)^*)$ is a transition invariant for $\trn$.
\end{theorem}

\nop{
Loop summarization is being recognized as an important tool in program analysis~\cite{conf/atva/KroeningSTTW08}.
Its potential for termination and bound analysis has been first recognized in~\cite{conf/pldi/GulwaniZ10}, and more recently in~\cite{conf/tacas/TsitovichSWK11}.
Loop summaries can be seen as a special case of procedure summaries, e.g.~\cite{conf/esop/GulwaniT07}.
}

%\begin{lemma}
%  Let $\transinv$ be a transition set.
%  We have $\bigcup \transinv^* \subseteq \bigcup \gamma(\alpha(\transinv)^*)$.
%\end{lemma}
%\begin{proof}
%  We have to show $\bigcup \transinv^* \subseteq \bigcup \gamma(\alpha(\transinv)^*)$.
%  We first show that $\trn_1 \circ \cdots \circ \trn_k \subseteq \gamma(\alpha(\trn_1) \circ \cdots \circ \alpha(\trn_k))$ for all $k \ge 0, \trn_1,\ldots,\trn_k \in \transinv$.
%  Let $k \ge 0$ be some integer and $trn_1,\ldots,\trn_k \in \transinv$ some transitions.
%  We have $\trn_i \subseteq \gamma(\alpha(\trn_i))$ for all $1 \le i \le k$ by the properties of a Galois connection.
%  Thus $\trn_1 \circ \cdots \circ \trn_k \subseteq \gamma(\alpha(\trn_1)) \circ \cdots \circ \gamma(\alpha(\trn_k))$.
%  Because $\alpha$ is monotone, we have $\alpha(\trn_1 \circ \cdots \circ \trn_k) \subseteq \alpha(\gamma(\alpha(\trn_1)) \circ \cdots \circ \gamma(\alpha(\trn_k)))$.
%  By the definition of concatenation of SCRs, we get $\alpha(\trn_1 \circ \cdots \circ \trn_k) \subseteq \alpha(\trn_1) \circ \cdots \circ \alpha(\trn_k)$.
%  This gives us $\trn_1 \circ \cdots \circ \trn_k \subseteq \gamma(\alpha(\trn_1)) \circ \cdots \circ \alpha(\trn_k))$ by the properties of a Galois connection.\\
%
%  $ \bigcup \gamma(\alpha(\transinv)^* =
%    \bigcup \gamma(\bigcup_{k \ge 0} \alpha(\transinv)^k) =
%    \bigcup \bigcup_{k \ge 0} \gamma(\alpha(\transinv)^k) = \\
%    \bigcup_{k \ge 0} \bigcup \gamma(\alpha(\transinv)^k) = \bigcup_{k \ge 0} \bigcup \{ \gamma(\alpha(\trn_1) \circ \cdots \circ \alpha(\trn_k)) \mid \trn_1,\ldots,\trn_k \in \transinv\} = \bigcup_{k \ge 0, \trn_1,\ldots,\trn_k \in \transinv} \gamma(\alpha(\trn_1) \circ \cdots \circ \alpha(\trn_k)) \supseteq \bigcup_{k \ge 0, \trn_1,\ldots,\trn_k \in \transinv} \trn_1 \circ \cdots \circ \trn_k = \bigcup_{k \ge 0} \bigcup \{ \trn_1 \circ \cdots \circ \trn_k  \mid \trn_1,\ldots,\trn_k \in \transinv\} = \bigcup_{k \ge 0} \bigcup \transinv^k = \bigcup \bigcup_{k \ge 0} \transinv^k = \bigcup \transinv^*. $
%\end{proof}

%Of particular interest are idempotent SCRs and transitions.
%\begin{definition}
%  An SCR $\scr$ is \emph{idempotent}, if $\scr \circ \scr = \scr$.
%  A transition $(\loc_1,\scr,\loc_2)$ is \emph{idempotent}, if $\scr$ is idempotent and $\loc_1 = \loc_2$.
%\end{definition}

%Next we introduce some useful notation.
%Considering an SCS $\scs$, we use $\sclocs^\scs$ to refer to its set of locations, $\scvars^\scs$ to refer to its set of variables, and $\rightarrow^\scs$ to refer to its set of transitions.
%Furthermore we identify $\scs$ with its set of transitions $\rightarrow^\scs$, and we write $f_1 \xrightarrow{G} f_2 \in \scs$, instead of $f_1 \xrightarrow{G} f_2 \in \Edges^\scs$.

%Importantly, the termination problem of SCR sets is decidable in PSPACE~\cite{conf/popl/LeeJB01,mcs-integers} and ranking functions can be constructed~\cite{mcs-integers,journals/corr/abs-0903-4382}.

\nop{
\begin{theorem}[\cite{conf/popl/LeeJB01,mcs-integers}]
\label{thm:scs-termination}
%  An SCS $\scs$ terminates, if for every idempotent transition $(\loc,\scr,\loc)$ of $\scs^+$ there is a norm $\norm \in \norms$ with $\norm > \norm^\prime \in \scr$. This can be decided in PSPACE.
Termination of SCS is decidable in PSPACE.
\end{theorem}

\noindent For the construction of SCS ranking functions we refer to~\cite{mcs-integers,journals/corr/abs-0903-4382}.
} 

==> include/rankings.tex <==
\section{Heuristics for Extracting Norms}
\label{sec:heuristics}

In this section we describe our heuristic for extracting norms from programs.
Let $\prog = (\locs,\edges)$ be a program and $\loc \in \locs$ be a location.
We compute all cycle-free paths from $\loc$ back to $\loc$.
For all arithmetic conditions $x \ge y$ appearing in some of these paths we take $x-y$ as a norm if $x-y$ decreases on this path; this can be checked by an SMT solver.
Note that in such a case $x-y$ is a local ranking function for this program path.
Similar patterns and checks can be implemented for iterations over bitvectors and data structures.
For a more detailed discussion on how to extract the local ranking functions of a program path we refer the reader to~\cite{conf/pldi/GulwaniZ10}.
We also compute norms for inner loops on which already extracted norms are control dependent and add them to the set of norms until a fixed point is reached (similar to program slicing).
We also include the sum and the difference of two norms, if an inner loop affects two norms at the same time.
Further, we include the rounded logarithm of a norm, if the norm is multiplied by a constant on some program path.
In general any integer-valued expression can be used as a program norm, if considered useful by some heuristic.
Clearly the analysis gets more precise the more norms are taken into account, but also more costly.

%An alternative to the pattern based approach for arithmetic progress measures is to use more involved methods such as~\cite{conf/vmcai/PodelskiR04}.
%We mention two approaches for handling complex data structures whose norms are not captured by the patterns in Section~\ref{sec-ranking}:
%\begin{itemize}
%\item One could preanalyze common data structures (such as provided in standard libraries) and provide a set of norms for them.
%    This approach achieves a separation of concerns between analyzing  application code and library functions.
%\item If this is not possible, one could automatically abstract such data structures before the actual analysis and derive an integer program using techniques such as as~\cite{conf/popl/GulwaniLS09,conf/popl/MagillTLT10}.
%\end{itemize} 

==> include/related.tex <==
\vspace{-0.3cm}
%\section{Related Work (More in Appendix~\ref{sec:comparison})}
\section{Related Work}
\label{sec:related}
\vspace{-0.2cm}
In recent work~\cite{conf/sas/HeizmannJP10} it was shown that SCA~\cite{conf/popl/LeeJB01,mcs-integers} is an instance of the more general technique of transition predicate abstraction (TPA)~\cite{conf/popl/PodelskiR05}.
We argue that precisely because of its limited expressiveness SCA is suitable for bound analysis: abstracted programs are simple enough such that we can compute bounds for them.
While we describe how to make imperative programs amenable to bound analysis by SCA, \cite{conf/sas/HeizmannJP10} is not concerned with practical issues.
%
The {\sc Terminator} tool~\cite{conf/pldi/CookPR06} uses TPA for constructing a Ramsey based termination argument~\cite{conf/lics/PodelskiR04}.
This argument does not allow to construct ranking functions or bounds from termination proofs and requires reasoning about the transitive hulls of programs by a software model checker, which is the most expensive step in the analysis.
Our light-weight static analysis uses SCA for composing global bounds from bounds on norms and requires only the computation of transitive hulls of abstracted programs, which is markedly less expensive.
%
Recent papers~\cite{conf/cav/KroeningSTW10,conf/tacas/TsitovichSWK11} propose to construct abstract programs for which termination is obvious and which are closed under transitivity in order to avoid analyzing transitive hulls of programs.
%Unfortunately the effectiveness of the algorithm in~\cite{conf/cav/KroeningSTW10} is limited (cf. Section~\ref{subsec:loopfrog} of the appendix). ~\cite{conf/tacas/TsitovichSWK11}
%
Others~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07} propose to lift standard abstract domains (as octagon, polyhedra) to powerset domains for the computation of disjunctive transition invariants, which requires a difficult lifting of the widening operator.
In contrast, SCA is a finite powerset abstract domain, which can handle disjunction but does not require widening.
%
In earlier work~\cite{conf/pldi/GulwaniZ10} we stated ad hoc proof rules for computing global bounds from local bounds of transitions.
We generalize these rules by our bound algorithm and identify SCA as a suitable abstraction for bound analysis.
Our contextualization technique is a sound generalization of the flawed \emph{enabledness check} of~\cite{conf/pldi/GulwaniZ10}.
%
Like our paper, \cite{conf/pldi/GulwaniJK09} proposes the use of program transformation for bound analysis.
While the algorithm of~\cite{conf/pldi/GulwaniJK09} is involved and parameterized by an abstract domain, our program transformations are easy to implement and rely only on an SMT solver.
%
Despite its success in functional/declarative languages, e.g.~\cite{conf/cav/ManoliosV06,conf/cade/Krauss07}, SCA~\cite{conf/popl/LeeJB01,mcs-integers} has not yet been applied to imperative programs.
We are the first to describe such an analysis.
%
%
%A series of works describes a type-based potential-method of amortized analysis for the estimation of resource usage in first-order functional programs, which reduces the problem to linear constraint solving, e.g.~\cite{conf/popl/HoffmannAH11,conf/popl/JostHLH10}.
%%
%Research on worst case execution time (WCET) estimation~\cite{journals/tecs/WilhelmEEHTWBFHMMPPSS08}
%either requires user annotation for bounding the number of loop iterations or employs simple techniques based on pattern matching and numerical analysis.
%

We give a detailed comparison with the cited approaches and others in the extended version.
%Section~\ref{sec:comparison} of the appendix.

%\section{Related Work}
%
%Recent work~\cite{conf/sas/HeizmannJP10} has shown that classical SCA~\cite{conf/popl/LeeJB01,mcs-integers} is an instance of transition predicate abstraction (TPA)~\cite{conf/popl/PodelskiR05}.
%While we find this fact quite intuitive (our analysis is also an instance of TPA), we are concerned with the opposite statement: precisely because the expressiveness of SCA is limited, bound analysis can be done on abstracted programs.
%Whereas we describe how to make SCA amenable to general imperative programs by using appropriate program transformations, \cite{conf/sas/HeizmannJP10} compares SCA and TPA on imperative programs derived from tail-recursive functional programs and is entirely ignorant of practical issues.
%
%The {\sc Terminator} tool~\cite{conf/pldi/CookPR06} uses TPA for constructing a Ramsey based termination argument~\cite{conf/lics/PodelskiR04}.
%The Ramsey argument has the disadvantage that global ranking functions or bounds cannot be extracted from termination proofs and that it requires reasoning about the transitive hulls of programs, which is the most expensive step of the analysis.
%In contrast, our approach uses SCA for composing global bounds from bounds on norms and requires only the computation of transitive hulls of abstracted programs, which is inexpensive.
%{\sc Terminator} relies on a full-fledged software model checker that implements the CEGAR loop,
%whereas our analysis is a simple and light-weight static analysis that relies only on an SMT solver.
%
%\cite{conf/cav/KroeningSTW10} proposes to construct abstract programs for which termination is obvious and which are closed under transitivity in order to avoid analyzing transitive hulls of programs as required in TPA based analyses like {\sc Terminator}~\cite{conf/pldi/CookPR06}.
%\cite{conf/cav/KroeningSTW10} gives an iterative algorithm which unfortunately does not work for principal reasons (cf. Section~\ref{subsec:loopfrog} of the appendix).
%We view our analysis as a rectification of~\cite{conf/cav/KroeningSTW10}, because it abstracts programs with SCA such that termination is preserved.
%
%The bound and termination analyses~\cite{conf/pldi/GulwaniZ10,conf/popl/BerdineCCDO07} propose to lift standard abstract domains (as octagon, polyhedra) to powerset domains for the computation of disjunctive transition invariants.
%\cite{conf/pldi/GulwaniZ10} states an algorithm for lifting the widening operator, which is quite involved, and not all implementation details are given.
%\cite{conf/popl/BerdineCCDO07} does not even explain how to lift the widening operator and remains vague on the implemented widening.
%In contrast SCA is a finite powerset abstract domain.
%This has the advantage, that we do not require complicated widening procedure, but that at the same time we can handle disjunction precisely.
%
%In earlier work~\cite{conf/pldi/GulwaniZ10} we stated proof rules for computing global bounds from local bounds of transitions.
%In this paper we have identified SCA as a suitable abstraction for bound analysis, which generalizes all the proof rules of~\cite{conf/pldi/GulwaniZ10} and which offers a general framework in which the bound problem can be placed.
%In~\cite{conf/pldi/GulwaniZ10} we stated a so-called \emph{enabledness} check that detects non-interference between transitions.
%Unfortunately, this check is flawed.
%Our program transformation contextualization provides a sound way of inferring non-interference.
%\cite{conf/pldi/GulwaniJK09} likewise proposes to use program transformation before performing bound analysis.
%Whereas the algorithm of~\cite{conf/pldi/GulwaniJK09} is involved and parameterized by an abstract domain, which is not further specified, our program transformations are easy to implement and rely only on an SMT solver.
%
%Despite its success in functional/declarative languages, e.g.~\cite{conf/cav/ManoliosV06}, \cite{conf/cade/Krauss07}, SCA~\cite{conf/popl/LeeJB01,mcs-integers} has not yet been applied to imperative programs.
%We believe that applying program transformations and choosing the local progress measures as size-change variables are essential steps for making imperative programs amenable to SCA.
%
%A series of works describes a type-based potential-method of amortized analysis for the estimation of resource usage in first-order functional programs, which reduces the problem to linear constraint solving, e.g.~\cite{conf/popl/HoffmannAH11,conf/popl/JostHLH10}.
%%Recent enhancement includes the extension to multivariate polynomial bounds~\cite{conf/popl/HoffmannAH11} and higher-order programs~\cite{conf/popl/JostHLH10}.
%
%Research on worst case execution time (WCET) estimation~\cite{journals/tecs/WilhelmEEHTWBFHMMPPSS08}
%either requires user annotation for bounding the number of loop iterations or employs simple techniques based on pattern matching and numerical analysis.
%
%We give a detailed comparison with the cited approaches in Section~\cite{sec:comparison} of the appendix. 

==> include/transformation.tex <==
%Abstracting a single transition on its own is not precise enough in most of the cases.
%Consider for example the two consecutive transitions {\tt i++;i--}.
%By abstracting them separately we loose all information because abstracting {\tt i++} results in $i < i^\prime$ and abstracting {\tt i--} results in $i^\prime > i^{\prime\prime}$, which combined results in no relation between $i$ and $i^{\prime\prime}$.
%However, by abstracting the two transitions jointly we obtain the identity relation $i = i^{\prime\prime}$.

%As explained in the example Section~\ref{subsec:example-abstraction} it is beneficial to concatenate a transition with its consecutive transitions.
%%We formally define concatenation following Manolios and Vroon~\cite{conf/cav/ManoliosV06}.
%
%\begin{definition}[Concatenation]
%  Let $\prog = (\locs, \edges)$ be a program and let $e = (\loc_1,\trn,\loc_2) \in \edges$ be a transition.
%  The result of \emph{concatenating} $e$ is the program $\prog^\prime = (\locs,\edges^\prime)$, where
%  \begin{displaymath}
%    \edges^\prime = (\edges \setminus e) \bigcup_{(\loc_2, \trn^\prime, \loc_3) \in \edges}(\loc_1,\trn \circ \trn^\prime,\loc_3).
%  \end{displaymath}
%\end{definition}
%
%If we assume that transitions relations are given as conjunctions of logical formulae,
%the concatenation of two transition relations can be implemented by conjoining their formulae and adequately substituting the intermediate variables by fresh variables.

%\begin{proposition}
%\label{prop:concatenation-correctness}
%  Let $\prog$ be a program and let $\prog^\prime$ be the program after the concatenation of some transition.
%  $\prog$ is terminating iff $\prog^\prime$ is terminating.
%  Furthermore $\prog$ and $\prog^\prime$ have the same complexity.
%  \TODO{make the complexity claim precise}
%\end{proposition}
%
%Recent developments in program analysis have shown that is beneficial to
%abstract large pieces of a program jointly rather than single transitions~\cite{conf/pldi/GulwaniZ10,conf/fmcad/BeyerCGKS09}.
%
%A crucial notion for contracting single transitions into larger ones is the notion of cutpoints, which is used throughout the literature.
%We give a definition of cutpoints here and show how they can be used for contracting transitions in program.
%We will see later how cutpoints can be used when abstracting the program.
%
%\begin{definition}[Cutpoints]
%  Let $\prog = (\locs, \edges)$ be a program.
%  A set of \emph{cutpoints}  $C \subseteq \locs$ is a subset of the locations such that the CFG of $\prog$ after having deleted all vertices of $C$ and all edges to which a vertex of $C$ is incident is acyclic.
%  %, i.e., the graph $G = (\locs \setminus C, \edges \setminus \{ (\loc_1,\trn,\loc_2) \in \edges \ | \ \loc_1 \in C \text{ or } \loc_2 \in C\})$ is acyclic.
%\end{definition}

%Given a set of cutpoints $C$ we transform a program as follows: for every program path between two cutpoints such that there is no further cutpoint on this path we contract the path to a single transition.
%
%\begin{definition}[Cutpoint Contraction]
%  Let $\prog = (\locs, \edges)$ be a program and let $C$ be a set of cutpoints of $\prog$.
%  The \emph{cutpoint contraction} of $\prog$ w.r.t. $C$ is the program $P^\prime = (\locs^\prime,\edges^\prime)$, where
%  \begin{itemize}
%  \item $\locs^\prime = C$, and
%  \item $\edges^\prime = \bigcup_{\loc_1, \loc_k \in C, l_i \in \locs \setminus C \text { for } 1 < i < k} \{(\loc_1,\trn_1 \circ \cdots \circ \trn_{k-1},\loc_k) \mid \text{ there are } (\loc_i,\trn_i,\loc_{i+1}) \in \edges \text{ for all } 1 \le i < k\}$.
%  \end{itemize}
%\end{definition}
%Note that a cutpoint contraction is just a series of concatenations.

%If we assume that transitions relations are given as conjunctions of logical formulae,
%the cutpoint contraction conjoins all transition relations on a program path in the same way as explained in the previous subsection.

%\begin{corollary}
%\label{prop:cutpoint-contraction-correctness}
%  Let $\prog$ be a program and let $\prog^\prime$ be the program after the contraction of some set of cutpoints.
%  $\prog$ is terminating iff $\prog^\prime$ is terminating.
%  Furthermore $\prog$ and $\prog^\prime$ have the same complexity.
%  \TODO{make the complexity claim precise}
%\end{corollary}
%\begin{proof}
%  As every cutpoint contraction consists of a series of concatenations the claim on termination and complexity follows from Proposition~\ref{prop:concatenation-correctness}.
%  All locations that are not cutpoints are not reachable after all possible edges have been concatenated, and can therefore be deleted from the program.
%\end{proof}


\subsection{Unrolling}
\label{subsec:unrolling}

\hv{First sentence does not connect to the text}

\todo{Cite Sumit's work \cite{conf/popl/GulwaniMT08}}

We argue that SCA is the right abstraction for the termination / bound problem, because keeping track of the monotonic changes of norms is sufficiently precise.
A problem arises when the monotonic increase or decrease of a norm establishes itself only after some iterations.
An example for such a behavior is a loop with counter $i$ that increments $i$ and decrements $i$ by 2 alternatingly.
In such a case abstraction of every path from the loop header back to the header is too imprecise.
For the example this would result in the predicates $i < i'$ and $i>i'$, which is too imprecise.
However, SCA is sufficiently precise, if two iterations of the loop are abstracted jointly.
A systematic way for abstracting a fixed number of loop iterations jointly, is to unroll the loop or parts of it before the actual abstraction is done.

\begin{definition}[Unrolling]
  Let $\transinv$ be a transition set, and let $(\mathit{next},\mathit{exit}) = \mathtt{Unroll}(\transinv)$ be some return value of Algorithm~\ref{alg:unrolling}.
  The pair of transition sets $(\mathit{next},\mathit{exit})$ is called an \emph{unrolling} of $\transinv$.
\end{definition}

\begin{algorithm}
\KwIn{transition set $\transinv = \{\trn_1,\ldots,\trn_n\}$}
\KwOut{looping transitions $\mathit{next}$, exit transitions $\mathit{exit}$}
\SetKwFunction{Choose}{choose}
\SetKwFunction{Heuristic}{heuristic}
$\mathit{next} := \transinv$; $\mathit{exit} := \{Id\}$\;
\While{$\trn := \Choose(\mathit{next})$}{
  $\mathit{next} := \mathit{next} \setminus \{\rho\} \cup \{\trn \circ \trn_1, \ldots, \trn \circ \trn_n\}$\;
  $\mathit{exit} := \mathit{exit} \cup \{\trn\}$\;
}
\Return $(\mathit{next},\mathit{exit})$\;
\caption{{\tt Unroll} computes unrollings}
\label{alg:unrolling}
\end{algorithm}

\begin{lemma}
  Algorithm~\ref{alg:unrolling} maintains the invariant $\mathit{next}^* \circ \mathit{exit} = \transinv^*$.
\end{lemma}

\hv{In the algorithm, choose is unclear. Also, termination should be discussed.}


%\begin{corollary}
%\label{prop:unrolling-correctness}
%  Let $\prog$ be a program and let $\prog^\prime$ be an unrolling of $\prog$.
%  $\prog$ is terminating iff $\prog^\prime$ is terminating.
%  Furthermore $\prog$ and $\prog^\prime$ have the same complexity.
%  \TODO{make the complexity claim precise}
%\end{corollary}
%\begin{proof}
%  As every unrolling consists of a series of concatenations the claim on termination and complexity follows from Proposition~\ref{prop:concatenation-correctness}.
%\end{proof}

Note that Algorithm~\ref{alg:unrolling} is parameterized by a function {\tt choose} that
heuristically chooses an element for further unrolling or stops the unrolling.
%
For example consider the inner loop $\prog = \{\loc_2; \rho_2,\rho_3\}$ in Ex.~\ref{ex:abstraction}.
An unrolling of $\prog$ is the program $\prog^\prime = \{\{\loc,\loc^\prime\},\{\loc \xrightarrow{\trn_2 \circ \trn_2} \loc, \loc \xrightarrow{\trn_2 \circ \trn_3} \loc, \loc \xrightarrow{\trn_3 \circ \trn_2} \loc, \loc \xrightarrow{\trn_3 \circ \trn_3} \loc \cup \{\loc \xrightarrow{Id} \loc^\prime, \loc \xrightarrow{\trn_2} \loc^\prime,\ \loc \xrightarrow{\trn_3} \loc^\prime\}\}$, where
$\trn_2 \circ \trn_2 = \trn_3 \circ \trn_3 = \mathit{false}$ and $\trn_2 \circ \trn_3 = \trn_3 \circ \trn_2 = a > 0 \wedge  a^\prime = a - 1 \wedge b^\prime = b + 1 \wedge \mathit{flag}^\prime = \mathit{flag}$.

We demonstrate the power of unrolling in combination with SCA for the termination analysis of an example from the literature.
In \cite{conf/popl/PodelskiR05} Podelski and Rybalchenko demonstrate the strength of their analysis on the program {\tt choice} that exemplifies how transition predicate abstraction can be used with transition systems to prove the termination of an example that cannot be proven by a lexicographic ranking function based on the ranking functions $x$, $y$ and $x+y$.
Their program {\tt choice} $\prog$ consists of two transitions:

\smallskip

{\small
\noindent $\trn_1 \equiv x > 0 \wedge y > 0 \wedge x^\prime = x-1 \wedge y^\prime = x$\\
$\trn_2 \equiv x > 0 \wedge y > 0 \wedge x^\prime = y-2 \wedge y^\prime = x+1$
}

\smallskip

\noindent Abstracting $\prog$ directly to a size-change program results in the size-change relations $\scr_1$ and $\scr_2$ that are not sufficient to prove program termination:

\smallskip

{\small
\noindent$\scr_1 \equiv x > 0 \wedge y > 0 \wedge x^\prime < x \wedge y^\prime = x$\\
$\scr_2 \equiv x > 0 \wedge y > 0 \wedge x^\prime < y \wedge y^\prime > x$
}

\smallskip

\noindent We unroll the transition labeled by $\trn_2$ and obtain the program $\prog^\prime = \{\{\loc,\loc^\prime\}, \{\loc \xrightarrow{\trn_1} \loc, \loc \xrightarrow{ \trn_2 \circ \trn_1} \loc, \loc \xrightarrow{\trn_2 \circ \trn_2} \loc\} \cup \{\loc \xrightarrow{Id} \loc, \loc \xrightarrow{\trn_2} \loc\}$.
As the location $\loc^\prime$ is not relevant for termination analysis we investigate only the simple loop $\prog^{\prime\prime} = \{\loc;\trn_1,\trn_2 \circ \trn_1, \trn_2 \circ \trn_2\}$, where

\smallskip

{\small
\noindent $\trn_1 \equiv x > 0 \wedge y > 0 \wedge x^\prime = x-1 \wedge y^\prime = x$\\
$\trn_2 \circ \trn_1 \equiv x > 0 \wedge y > 0 \wedge x^\prime = y-3 \wedge y^\prime = y-2$\\
$\trn_2 \circ\trn_2 \equiv x > 0 \wedge y > 0 \wedge x^\prime = x-1 \wedge y^\prime = y-1$
}

\smallskip

\noindent Size-change abstracting these transition relations results in:

\smallskip

{\small
\noindent $\scr_1 \equiv x > 0 \wedge y > 0 \wedge x^\prime < x \wedge y^\prime = x$\\
$\scr_{21} \equiv x > 0 \wedge y > 0 \wedge x^\prime < y \wedge y^\prime < y$\\
$\scr_{22} \equiv x > 0 \wedge y > 0 \wedge x^\prime < x \wedge y^\prime < y$
}

\smallskip

\noindent By the main result of~\cite{mcs-integers} this suffices to prove termination.

\smallskip

Since unrolling happens before the abstraction is computed, it increases the precision of all subsequent steps.
%In practice we first perform an analysis without unrolling and if this fails we try to unroll the parts of the loops once

%In practice we unroll loops once it the abstraction without unrolling results %in conflicting progress measures on two transitions.


